MoDora: Tree-Based Semi-Structured Document Analysis System

Semi-structured documents integrate diverse interleaved data elements (e.g., tables, charts, hierarchical paragraphs) arranged in various and often irregular layouts. These documents are widely observed across domains and account for a large portion of real-world data. However, existing methods struggle to support natural language question answering over these documents due to three main technical challenges: (1) The elements extracted by techniques like OCR are often fragmented and stripped of their original semantic context, making them inadequate for analysis. (2) Existing approaches lack effective representations to capture hierarchical structures within documents (e.g., associating tables with nested chapter titles) and to preserve layout-specific distinctions (e.g., differentiating sidebars from main content). (3) Answering questions often requires retrieving and aligning relevant information scattered across multiple regions or pages, such as linking a descriptive paragraph to table cells located elsewhere in the document. To address these issues, we propose MoDora, an LLM-powered system for semi-structured document analysis. First, we adopt a local-alignment aggregation strategy to convert OCR-parsed elements into layout-aware components, and conduct type-specific information extraction for components with hierarchical titles or non-text elements. Second, we design the Component-Correlation Tree (CCTree) to hierarchically organize components, explicitly modeling inter-component relations and layout distinctions through a bottom-up cascade summarization process. Finally, we propose a question-type-aware retrieval strategy that supports (1) layout-based grid partitioning for location-based retrieval and (2) LLM-guided pruning for semantic-based retrieval. Experiments show MoDora outperforms baselines by 5.97%-61.07% in accuracy. The code is at https://github.com/weAIDB/MoDora.

==> response.tex <==
%\noindent \textbf{\Large Dear Meta-Reviewer and Reviewers,}

\noindent We thank all reviewers for their thoughtful reviews and encouraging comments. We have carefully revised our paper as suggested. We will respond to each reviewer's comment below,  pointing to changes we made in our revised paper, in \RaColor{blue (for \hyperlink{R1.O1}{\emph{Reviewer \#1}})}, \RbColor{orange (for \hyperlink{R2.O1-(1)}{\emph{Reviewer \#2}})}, and \RcColor{red (for \hyperlink{R3.O1}{\emph{Reviewer \#3}})}, respectively. 

% \noindent Thanks for your thoughtful reviews and encouraging comments. We have significantly improved the manuscript by strictly following all revision requests.
% Revisions made in response to three reviewers are highlighted in \RaColor{blue (for \hyperlink{R1.O1}{\emph{Reviewer \#1}})}, \RbColor{orange (for \hyperlink{R2.O1}{\emph{Reviewer \#2}})}, and \RcColor{red (for \hyperlink{R3.O1}{\emph{Reviewer \#3}})}, respectively.



\section*{Response to Meta-Reviewer}
% \begin{table}[h]
% \vspace{-.3cm}
% \caption{Revision Summary for Meta-Reviewer.}
% \vspace{-.35cm}
% \label{tab:reviewer2}
% \resizebox{.95\linewidth}{!}{
% \begin{tabular}{c|l|c}
% \hline
% \textbf{ID} & \multicolumn{1}{c|}{\textbf{Revision Items}} & \textbf{Requests} \\ \hline
% \textbf{1}  & Add important related works like  LayoutLMv3 and DocFormer.  & Meta.O1 \\ \hline
% \textbf{2}  & Adding experiments with additional benchmarks and baselines. & Meta.O2 \\ \hline
% \textbf{3}  & Discuss designs of parsing tools and tree structure in more detail. & Meta.O3 \\ \hline
% \end{tabular}
% }
% \vspace{-.25cm}
% \end{table}

%added the \xbr{five important} related works in Section~\ref{sec:intro} and Section~\ref{subsec:relatedwork}.

%\yeye{if we could not shorten our responses for R1/R2/R3 to fit in 4 pages, can consider shorten our response for meta-reviewer, by only pointing out the changes we made (Line xxx, Table yyy), and ask meta-reviewer to check RX.OY instead of repeating content here.}


\begin{shaded*}
%\noindent\textbf{Meta.Overall.} We invite you to submit a revised version of the paper, based on your revision plan. Make sure to integrate all revision requests raised by the reviewers, including but not limited to:
%\vspace{.5em}

\noindent \hypertarget{Meta.O1}{\textbf{Meta.O1.}} Expanding the related work section (e.g., R1.O3). %\xbr{sync with R1.O3 and main text}% Related work misses important contributions such as LayoutLMv3, DocFormer.
\end{shaded*}

\noindent \textbf{Response:} %Thanks for the valuable suggestion. 
We have substantially expanded our discussions on related work, such as DocFormer~\cite{appalaraju2021docformer} and LayoutLMv3~\cite{huang2022layoutlmv3} 
in \lspref{more_work1} and \lspref{more_work2}, in response to \emph{\hyperlink{R1.O3}{R1.O3}}.  We have also added  dicussions of related work on document analysis methods in our revised \lspref{more_work3}, including ZenDB \cite{zendb}, DocAgent~\cite{sun2025docagent}, SuperRAG~\cite{yang2025superrag},  PDFTriage~\cite{saad2024pdftriage} in response to \emph{\hyperlink{R2.O1-(1)}{R2.O1-(1)}} and \emph{\hyperlink{R2.O1-(2)}{R2.O1-(2)}}. 
%DocFormer~\cite{appalaraju2021docformer} and LayoutLMv3~\cite{huang2022layoutlmv3} are page-level document understanding models that input page images and OCR-extracted text and encode them using multimodal Transformers. However, both models primarily capture local and sequential relationships among document elements and lack explicit modeling of higher-level document structures, such as cross-block hierarchies and inter-section organization. Moreover, their limited model scale and maximum sequence length (e.g., 512 text tokens in LayoutLMv3) make it difficult to process lengthy or multi-page documents. 

%, which restricts their effectiveness in tasks like \zxh{replace with a specific case (e.g., )}.

% \begin{MetaBox}
% \lspref{more_work1} 
% (4) End-to-End models including pre-trained models and Multimodal Large Language Models (MLLMs), such as LayoutLMv3~\cite{huang2022layoutlmv3}, DocFormer~\cite{appalaraju2021docformer} ... %UDOP~\cite{tang2023unifying}, DocOwl2~\cite{hu2024mplug} and GPT-5~\cite{openai2025gpt5}, can directly process documents. But they tend to overlook fine-grained contents and layout relationships when the input length grows, leading to incomplete reasoning. 
% \end{MetaBox}

%This arises from their limitations in understanding complex document structures and adapting to multi-page documents.
% LayoutLMv3 (while DocFormer is an earlier work, and thus we mainly focus on comparing with the more recent LayoutLMv3)

\iffalse
\begin{MetaBox}
\lspref{more_work2}
%These models (e.g., LayoutLMv3~\cite{huang2022layoutlmv3}, DocFormer~\cite{appalaraju2021docformer},  UDOP~\cite{tang2023unifying}, DocOwl2~\cite{hu2024mplug}, and GPT-5~\cite{openai2025gpt5}) support end-to-end reasoning via pre-trained models or \llms. 
... DocFormer, LayoutLMv3, and UDOP input page-level document information (e.g., page images, OCR-parsed text, bounding boxes) directly into  %natively support page-level input. They take hybrid input like 
%image, OCR-parsed text and bbox, and transformer models based on their designed 
% discrete multi-modal encoder~\cite{appalaraju2021docformer}, word-patch alignment~\cite{huang2022layoutlmv3} and vision-text-layout unified encoder
pretrained transformer models. They primarily capture local and sequential relationships among document elements and lack explicit modeling of higher-level document structures, such as cross-block hierarchies and inter-section organization. Moreover, their limited model scale and maximum sequence length (e.g., 512 text tokens in LayoutLMv3) make it difficult to process lengthy or multi-page documents, which restricts their effectiveness on complex semi-structured document analysis tasks. %However, the model scale, maximum sequence length (e.g.  512 for text tokenization in LayoutLMv3) and the lack of high-level document structure modeling limit their analysis performances to semi-structured documents.
%... \zxh{add DocFormer} Although LayoutLMv3 is pre-trained with a word-patch alignment and is provided a hybrid input including the page image, OCR-parsed text and bbox, the model scale and embedding length limit its understanding of long context and elements correlations, leading to truncations and reasoning failures. UDOP also takes image+text+bbox input and applies a vision-text-layout transformer as unified encoder, but has similar limitations to LayoutLMv3. 

%Compared to the previous three tasks, DocOwl2 introduces high-resolution visual compression technique and apply a stronger LLM backbone. It supports multi-page input and achieves better performance, but still falls behind larger and more advanced MLLMs like GPT-5.
\end{MetaBox}
\fi

\iffalse
\begin{MetaBox}
\lspref{more_work2} 
On DUDE, for instance, LayoutLMv3 reaches 25.06 AIC-Acc and 23.43 ACNLS -- higher than models like UDOP, yet still far below MoDora's 83.70 and 77.24. A similar gap appears on MMDA, where LayoutLMv3 obtains 17.37 (AIC-Acc) and 13.96 (ACNLS), which are significantly lower than MoDora's 73.33 and 55.23. This arises from their limitations in understanding complex document structures and adapting to multi-page documents. \zxh{-- sync}
%These models (e.g., LayoutLMv3~\cite{huang2022layoutlmv3}, DocFormer~\cite{appalaraju2021docformer}, UDOP~\cite{tang2023unifying}, DocOwl2~\cite{hu2024mplug}, and GPT-5~\cite{openai2025gpt5}) support end-to-end reasoning via pre-trained models or \llms. DocFormer, LayoutLMv3 and UDOP natively support page-level input. They take hybrid input like image, OCR-parsed text and bbox, and train transformer models based on their designed discrete multi-modal encoder~\cite{appalaraju2021docformer}, word-patch alignment~\cite{huang2022layoutlmv3} and vision-text-layout unified encoder. However, the model scale, maximum sequence length (e.g.  512 for text tokenization in LayoutLMv3) and the lack of high-level document structure modeling limit their analysis performances to semi-structured documents. Compared to the previous three tasks, DocOwl2 introduces high-resolution visual compression technique and apply a stronger LLM backbone. It supports multi-page input and achieves better performance, but still falls behind larger and more advanced MLLMs like GPT-5.
\end{MetaBox}
\fi


%In addition, they are designed to support page-level input up to a limited length (e.g., with maximum length of 512 tokens), which can hardly process lengthy or multi-page documents. 

% are capable of encoding textual and visual information, they 
% restricts their straightforward extension to multi-page document processing.

%We have carefully added the related works. For end-to-end models (according to R1.O3), we have discussed LayoutLMv3 and DocFormer in both the related work section and main experiment.

%We have added discussions on related document QA works~\cite{huang2022layoutlmv3, appalaraju2021docformer, sun2025docagent, yang2025superrag, saad2024pdftriage}. 
%For pretrained models, LayoutLMv3 can \zxh{xxx}, but primarily models sequential relationships between document elements and struggles to capture higher-level document structures. DocFormer can \zxh{xxx} but \zxh{xxx}. 
%For structure extraction methods, they recognize the importance of tree structures, such as SHT and XML trees, for document modeling. But they overlook the capture of fine-grained location of document elements within page layouts, which can further strengthen the retrieval and answering.

%We appreciate this suggestion and have added corresponding discussion and experiments to highlight these important contributions.

%While both LayoutLMv3 and DocFormer can encode textual and layout information and thus perform document-related tasks, they have notable limitations. LayoutLMv3 . In addition, its model size restricts its capacity to handle long-range context in lengthy documents. The earlier baseline DocFormer suffers from similar limitations.

%\noindent $\bullet$ \textbf{(1) Introduction (Section~\ref{sec:intro}):}

%Besides, we have more diligently discussed seminal document analysis methods in \lspref{more_work3}, including ZenDB \cite{zendb}, DocAgent~\cite{sun2025docagent}, SuperRAG~\cite{yang2025superrag},  PDFTriage~\cite{saad2024pdftriage} (see \emph{\hyperlink{R2.O1}{R2.O1}}). 

%\xbr{They design various structures to capture the document structure and serve as retrieval base (e.g., semantic hierarchy tree in ZenDB, XML tree structure outline in DocAgent, layout-aware graph in SuperRAG and structured metadata in PDFTriage. But their parsing methods selection and node definitions ignore the alignment of textual data and bounding box of document elements at the tree/graph node level. That results in limitations or additional steps when processing non-digital documents or elements such as tables and charts.} %focusing on their limitations in \xbr{construction process and cross-modal analysis ability} .

\iffalse
\begin{MetaBox}
\lspref{more_work3}(2) Structure extraction methods like ZenDB~\cite{zendb} employ visual feature clustering and LLMs to extract partial document structures (e.g., distinguishing titles from body text), and raise a summarization mechanism to guide the search. But it fails on complex layouts, often misidentifying hierarchical levels and table regions, neither integrates the ability to process charts and images.
In addition, works such as DocAgent~\cite{sun2025docagent}, SuperRAG~\cite{yang2025superrag}, and PDFTriage~\cite{saad2024pdftriage} also employ structural documents modeling such as XML tree structure outline in DocAgent, layout-aware graph in SuperRAG and structured metadata in PDFTriage. However, due to the document parsing methods and node definitions, they also fail to align textual data and bounding box locations of document elements at the tree/graph node level. As a result, these approaches exhibit limitations or require additional steps when processing non-digital documents or elements such as tables and charts. %Furthermore, their retrieval mechanisms also vary—for instance, agent interaction, vector search and intermediate languages.
\end{MetaBox}
\fi

\begin{shaded*}
\noindent
\hypertarget{Meta.O2}{\textbf{Meta.O2.}} Adding experiments with additional benchmarks and baselines (last revision request by Reviewer 1; R3.O2)

% add experiments including MP-DocVQA / M3DocVQA

% It is necessary to add a baseline that just uses the extracted components to prompt the MLLM with the same retrieval strategies as the current approach (excluding the tree-based optimizations). This would help isolate whether the gains come from the element aggregation step that generates rich layout-aware components versus the tree-based approach itself.

\end{shaded*}

\begin{sloppypar}
\noindent \textbf{Response:} 
This is an important area of improvement. During revision, we have spent substantial efforts  adding both new benchmarks and baselines in our experiments.  Specifically, we have  now grown our benchmarks, from the two  we used in our original paper (DUDE and \ourbench), to a total of {7 benchmarks}, with the addition of MP-DocVQA and M3DocVQA as suggested in \emph{\hyperlink{R1.O5}{R1.O5}}, as well as Civic/Qasper/Contract as suggested in \emph{\hyperlink{R2.O1-(1)}{R2.O1-(1)}}.


Furthermore, we have added new baselines, including LayoutLMv3 (\emph{\hyperlink{R1.O3}{R1.O3}}), DocAgent (\emph{\hyperlink{R2.O1-(2)}{R2.O1-(2)}}), as well as many more ablation experiments (\emph{\hyperlink{R1.O4}{R1.O4}}, \emph{\hyperlink{R2.O3-(1)}{R2.O3}}, \emph{\hyperlink{R3.O2}{R3.O2}}). 

Encouragingly, across all these newly added benchmarks and baseline comparisons, \oursys consistently outperforms alternative methods, which we believe significantly strengthens the empirical evidence and overall contribution of the paper.

%We have updated the experiment results of LayoutLMv3 in {\emph{\textbf{Figure~\ref{fig:precompare}}}} for pilot study, as well as {\emph{\textbf{Figure~\ref{fig:trend}}}} and {\emph{\textbf{Table~\ref{tab:type}}}} in the main experiments (Section~\ref{sec:experiments}). On DUDE, LayoutLMv3 reaches 25.06 AIC-Acc and 23.43 ACNLS -- higher than models like UDOP, yet still far below MoDora's 83.70 and 77.24. A similar gap appears on MMDA, where LayoutLMv3 obtains 17.37 (AIC-Acc) and 13.96 (ACNLS), significantly lower than MoDora's 73.33 and 55.23. 

% We have added experiments on benchmarks MP-DocVQA and M3DocVQA in {\emph{\textbf{Figure~\ref{fig:trend}}}} and \lspref{main_discussion}. On MP-DocVQA, \oursys achieves 13\% accuracy compared to GPT-5, and 12\% on M3DocVQA. They further verify the benefits of \oursys's techniques, such as local-alignment aggregation for capturing inter-relationships among document elements (e.g., adjacent paragraphs sharing a title with specific reading order), semantic-locational hybrid retrieval strategy.

% We have added the baseline (\oursys w/o tree-based optimizations) as suggested in \emph{\hyperlink{R3.O2}{R3.O2}} (see {\emph{\textbf{Table~\ref{tab:ablation}}}} and \lspref{hi_ablation}). The results show a 15\% drop in accuracy on \ourbench and DUDE dataset, reflecting the importance of Component-Correlation Tree in modeling semi-structured documents.
\end{sloppypar}

%, its tree-based structure for organizing heterogeneous components, and its retrieval strategy that exploits both semantic and locational cues to improve recall and precision.

%We have updated Figure~\ref{fig:trend} in Section~\ref{sec:experiments} to include experimental results of additional benchmarks.

% On the MP-DocVQA and M3DocVQA datasets, \oursys achieves more than 78\% Accuracy

% \begin{MetaBox}
% \lspref{type_discussion} As shown in Table~\ref{tab:type}, \oursys achieves the best performance across all four question types defined in Section~\ref{subsec:questiontype}, demonstrating the effectiveness in capturing structural, textual, hybrid, and spatial information for document understanding...
% \end{MetaBox}

% \oursys without the tree-based optimizations shows a significant drop in quality (73.33 -> 59.25), (55.23 -> 45.85) for AIC-Acc and ACNLS on MMDA, and (83.70 -> 68.86) (77.24 -> 62.96) for the same on DUDE. %, which underlines the importance of the hierarchical representation in \oursys. 

 %These results have been added into Table~\ref{tab:ablation} and Section~\ref{subsec:ablation}.}

%\noindent \ding{182} First, we have added experiments using MP-DocVQA / M3DocVQA in the revised paper, as suggested.
%\end{sloppypar}

%\noindent $\bullet$ \textbf{Experiments (Section~\ref{sec:experiments}):} The experimental results have been included in the Section~\ref{sec:experiments}.


%\noindent \ding{183} Second, we have conducted the experiment of suggested baselines. There is 

%\noindent $\bullet$ \textbf{Ablation Study (Section~\ref{subsec:ablation}):} We have add the experimental results of the suggested baseline in Section~\ref{subsec:ablation}.

% \begin{MetaBox}
% \lspref{hi_ablation} 
% We isolate the impact of hierarchical representation via conducting question answering based on the flattened components with the same retrieval strategies. Without the assistance of tree structure, the AIC-Acc decreases greatly by -15.33\% and -15.49\% on DUDE and MoDora respectively. This demonstrates the utility of our structural modeling of CCTree.
% \end{MetaBox}

\begin{shaded*}
\noindent
\hypertarget{Meta.O3}{\textbf{Meta.O3.}} Discuss design decisions made by your approach in more detail (R1.O2; R3.O3)

% R1.O2: The method relies on OCR text and bounding boxes, while other signals typucally used by other approaches could help (e.g., native PDF structures, typographic cues)

% It is also necessary to discuss/show what is the size of the generated trees for real-world semi-structured documents. For the documents in the provided dataset, the generated trees do not seem too complex. The expensive tree-based approach seems unnecessary for these documents.

\end{shaded*}

\noindent \textbf{Response:}
We expanded our discussion on key design decisions:

%\noindent \ding{182} 
\textbf{OCR Instead of Native PDF Structures}: In response to R1.O2, we clarify that our use of OCR-based extraction is a deliberate design choice aimed at broad applicability to heterogeneous real-world documents. In practice, screenshots and scanned PDFs are common (e.g., accounting for approximately 20\% of documents in DUDE), yet lack native PDF metadata. OCR enables our system to handle these cases uniformly. We have added a more detailed discussion in \lspref{ocr_use}.

%\noindent \ding{183} 

\textbf{Tree-Based Structural Modeling}: In response to R3.O3, we expanded our discussion to clarify that our use of tree-based modeling for semi-structured documents is motivated by its ability to capture hierarchical relationships (e.g., heading levels), which are critical for downstream tasks such as summarization and retrieval.
To support this, we have added statistics in \emph{\textbf{Table~\ref{tab:datasets}}}. We further show that removing this  tree-based structure results in a 15 percentage point performance drop (in {\emph{\textbf{Table~\ref{tab:ablation}}}} of our revised paper), confirming its necessity in modeling semi-structured documents. %: DUDE yields an average of 17.2 nodes, 12.6 leaves, and 3.36 levels; MMDA benchmark shows greater complexity with 49.2 nodes, 37.7 leaves, and 4.23 levels. As discussed in Meta.O2, removing this  tree-based structure results in a 15\% performance drop. %confirming its necessity in modeling semi-structured documents.

%Our choice to use OCR was deliberate: it offers a generalizable approach that applies uniformly to the diverse real documents, including screenshots and scanned PDFs, where native PDF structures are not available (e.g., 20\% in DUDE). %{Experiment in Section~\ref{sec:sec:doc-preprocess} shows that parsing tools based on native PDF structures such as pymupdf~\cite{pymupdf} and pdfplumber~\cite{pdfplumber} encounter failures in many documents.}

% \noindent \ding{182} First, we emphasize that our choice to use OCR was deliberate: it offers a generalizable approach that applies uniformly to the diverse real documents, including screenshots and scanned PDFs, where native PDF structures are not available.

% \begin{MetaBox}
% \lspref{ocr_use} Here we choose OCR as the document-parsing tool, as it is a more versatile tool that can process both digital documents and raster-based documents (such as screenshots and scanned PDFs). We conduct a simple experiment to parse document using pymupdf~\cite{pymupdf} and pdfplumber~\cite{pdfplumber}, but they fail to parse some documents without native PDF structures. They are 20\% documents in DUDE~\cite{van2023document}, 10\% documents in our newly created dataset, and all PDFs of other two datasets~\cite{cho2024m3docrag, tito2023hierarchical} that are synthesized from our downloaded page images.
% \end{MetaBox}

%\noindent \ding{183} \xbr{The tree structure naturally captures hierarchical relationships within documents, such as heading levels. Building upon this structure, summarization generation and forward search further enable effective retrieval.} We also calculate some dataset statistics related to the tree. For example, in the DUDE dataset, the average tree size is 17.2 nodes, 12.6 leaves, and 3.36 levels; while in the new \oursys benchmark we created, the numbers are 49.2 nodes, 37.7 leaves, and 4.23 levels, respectively. \xbr{The ablation study in Meta.O2 has shown a 15\% drop without this structure, indicating the importance of tree representation in document modeling.}


%There is great complexity in documents in MMDA, and a tree structure is necessary to capture the complex layout. We have calculated the dataset statistics such as the tree size. For example, In the existing DUDE dataset, the average tree size is 17.2 nodes, 12.6 leaves, and 3.36 levels; while in the new MMDA benchmark we created, the numbers are 49.2 nodes, 37.7 leaves, and 4.23 levels, respectively. \zxh{rewrite}

% , making it a more challenging DocumentQA benchmark,

%\noindent $\bullet$ \textbf{Micro Benchmark Preparation(Section~\ref{ssec:bench}):} The dataset statistics such as the LD, ED, tree size and depth are reported in Section~\ref{ssec:bench} to prove the complexity of \ourbench and further indicate the necessity of tree construction.

% \begin{MetaBox}
% \lspref{dataset_ana} Existing datasets cannot well reflect the complexity of typical semi-structured document analysis tasks~\cite{tito2023hierarchical,cho2024m3docrag,van2023document}. The documents in MP-DocVQA~\cite{tito2023hierarchical} and DUDE~\cite{van2023document} exhibit limitations in content sufficiency, element richness and structural complexity. While M3DocVQA~\cite{cho2024m3docrag} are more challenging in these aspects, its documents are sourced from Wikipedia, lacking representativeness of other types of complex documents. Thus, in this section we introduce a new benchmark \oursys.

% \lspref{dataset_cmp} Besides, we compute various statistics for the four datasets, including the previously defined ED and LD, as well as the average number of nodes, leaves and levels of the CCTree constructed based on their documents. As shown in Table~\ref{tab:datasets}, \ourbench achieves optimal performance across most statistics, indicating its richer document element types, complexity of layout distribution, and sufficiency of content. \ourbench has fewer average CCTree levels than M3DocVQA, which is partly attributable to the fact that M3DocVQA consists of Wikipedia documents, which inherently possess more hierarchical title levels, whereas \ourbench also encompasses some document types with fewer heading levels.
% \end{MetaBox}


\begin{shaded*}
\noindent
\hypertarget{Meta}{\textbf{Meta.Overall.}} The revision plan is a good basis. Make sure to integrate all other requests raised by the reviewers, including the points mentioned above. 
\end{shaded*}

\noindent \textbf{Response:}  We have carefully revised the manuscript in accordance with the proposed revision plan and have also incorporated all additional requests and concerns raised by the reviewers. We kindly invite the meta-reviewer to refer to our responses to each reviewer comment below for details.
%key improvements are outlined below.

%We have thoroughly revised the whole paper based on the revision plan, with the major updates as follows:

% % Contribution \& 
% \noindent \ding{182} \textbf{Novelty Clarification:} %\noindent(1) We have clarified \xbr{the local-alignment aggregation rules are designed to integrate interrelated elements into components based on local layouts}, distinguishing them from parsing tools like OCR (for {\emph{\hyperlink{R1.O1}{R1.O1}}}).
% % the proposed local-alignment aggregation rules are designed to , not as MoDora's core contribution
% We have clarified that our focus lies in structural modeling, where we integrate interrelated elements into higher-level components based on local document layout cues. This is distinct from OCR parsing techniques, which we merely utilize as preprocessing tools (see \emph{\hyperlink{R1.O1}{R1.O1}}). We have (1) clarified that our structure extraction method is fundamentally distinct from prior approaches like SHT~[13] and (2) detailed how MoDora's fine-grained tree construction, information attenuation based summarization, node-level validation collectively contribute to its superior accuracy additionally on SHT's benchmark (for \emph{\hyperlink{R2.O1-(1)}{R2.O1}}).

%  % We have also clarified that our structure extraction method unifies text, tables and charts as nodes on CCTree and aligns their textual contents and bounding boxes

% %We have clarified that our focus lies in structural modeling, where the proposed local-alignment aggregation rules are designed to integrate interrelated elements into higher-level components based on local layout cues. This is distinct from document parsing techniques like OCR, which we merely utilize as preprocessing tools, not as \oursys's core contribution (see {\emph{\hyperlink{R1.O1}{R1.O1}}}).

% % the technical contributions that concentrate on document structural modeling and  question answering

% %\noindent(2) We have clarified that our structure extraction method unifies text, tables and charts as nodes on CCTree, align the textual contents and bboxes of them, and design a more comprehensive retrieval method based on the CCTree modeling. (for {\emph{\hyperlink{R2.O1}{R2.O1}}}).

% % We further strengthen the novelty of our system compared to other structure extraction methods, as it 

% \noindent \ding{183} \textbf{Datasets Comparison:} We have compared the statistics (e.g. LD, ED, tree nodes) of four datasets in detail, showing that MMDA is a more complex and challenging dataset, which has lower ED (0.264 compared to 0.305 of MP-DocVQA), higher LD (1.85 compared to 1.35 of DUDE) and more tree nodes (49.2 compared to 38.3 of M3DocVQA)  (for {\emph{\hyperlink{R1.O5}{R1.O5}}, \emph{\hyperlink{R3.O3}{R3.O3}}}).

% \noindent \ding{184} \textbf{Related Work Expansion:} We have added important related works, including end-to-end models like LayoutLMv3, DocFormer (for \emph{\hyperlink{R1.O3}{R1.O3}}), and structure extraction methods like DocAgent~\cite{sun2025docagent}, SuperRAG~\cite{yang2025superrag}, PDFTriage~\cite{saad2024pdftriage} (for \emph{\hyperlink{R2.O1}{R2.O1}}).

% %\noindent(1) We have added important related works, including end-to-end models like LayoutLMv3, DocFormer (for {\emph{\hyperlink{R1.O3}{R1.O3}}}), and structure extraction methods like DocAgent, SuperRAG, PDFTriage (for {\emph{\hyperlink{R2.O1}{R2.O1}}}).


% \noindent \ding{185} \textbf{Experiment Supplement:} We have added experiments of some baselines (LayoutLMv3 for \emph{\hyperlink{R1.O4}{R1.O4}}, DocAgent for \emph{\hyperlink{R2.O1}{R2.O1}}), datasets (MP-DocVQA and M3DocVQA for \emph{\hyperlink{R1.O5}{R1.O5}}, SHT's three datasets for \emph{\hyperlink{R2.O2}{R2.O2}}), cost study (for \emph{\hyperlink{R3.O1}{R3.O1}}) and ablation study (for \emph{\hyperlink{R1.O4}{R1.O4}}, \emph{\hyperlink{R3.O2}{R3.O2}}). We have also verified the effectiveness of the ACNLS metric (where full-document answers achieve only {43.85 on MMDA}) (for \emph{\hyperlink{R2.O3-(1)}{R2.O3-(1)}}). 

% % modified the metric of ACNLS to eliminate concerns that it would encourage long answers 

% %\noindent(1) We have added experiments of some related works \xbr{(for {\emph{\hyperlink{R1.O4}{R1.O4}}}, {\emph{\hyperlink{R2.O1}{R2.O1}}})}, datasets \xbr{(for {\emph{\hyperlink{R1.O5}{R1.O5}}}, {\emph{\hyperlink{R2.O2}{R2.O2}}})}, cost study \xbr{(for {\emph{\hyperlink{R3.O1}{R3.O1}}})} and ablation study  \xbr{(for {\emph{\hyperlink{R1.O4}{R1.O4}}}, {\emph{\hyperlink{R3.O2}{R3.O2}}})} . We also modify the metric of ACNLS to eliminate concerns that it will encourage long answers (for {\emph{\hyperlink{R2.O3-(1)}{R2.O3-(1)}}}).

% %(for {\emph{\hyperlink{R1.O4}{R1.O4}}}, {\emph{\hyperlink{R1.O5}{R1.O5}}}, {\emph{\hyperlink{R2.O1}{R2.O1}}}, {\emph{\hyperlink{R2.O2}{R2.O2}}}, {\emph{\hyperlink{R3.O1}{R3.O1}}}, {\emph{\hyperlink{R3.O2}{R3.O2}}})

% \noindent \ding{186} \textbf{Detail Clarification:} We have carefully explained the design decision of OCR usage (for \emph{\hyperlink{R1.O2}{R1.O2}}), realism of benchmark questions and evaluation of open-ended ones (for \emph{\hyperlink{R2.O3-(4)}{R2.O3-(4)}}), LLM's performance in question generation (for \emph{\hyperlink{R3.O4}{R3.O4}}) and captions/metadata generation (for \emph{\hyperlink{R3.O5}{R3.O5}}). We have also refined the description of parameter settings (for {\emph{\hyperlink{R2.O3-(2)}{R2.O3-(2)}}}), and ablation study setup (for {\emph{\hyperlink{R2.O3-(3)}{R2.O3-(3)}}}).

% %We have carefully explained the design decision of the use of OCR (for {\emph{\hyperlink{R1.O2}{R1.O2}}}), the scenario and evaluation of hierarchy questions (for {\emph{\hyperlink{R2.O3-(4)}{R2.O3-(4)}}}), the manual curation of questions (for {\emph{\hyperlink{R3.O4}{R3.O4}}}), and \llm's performance in captions/metadata generation (for {\emph{\hyperlink{R3.O5}{R3.O5}}}). We also refine the description of parameter and experiment settings to make them clear and avoid misunderstanding (for {\emph{\hyperlink{R2.O3-(2)}{R2.O3-(2)}}}, {\emph{\hyperlink{R2.O3-(3)}{R2.O3-(3)}}}).


%\vspace{-.75em}
\section*{Response to Reviewer \#1 \textcolor{blue}{(Blue)}}

\iffalse
\begin{table}[h]
\vspace{-.3cm}
\caption{Revision Summary for Reviewer \#1.}
\vspace{-.35cm}
\label{tab:reviewer2}
\resizebox{.95\linewidth}{!}{
\begin{tabular}{c|l|c}
\hline
\textbf{ID} & \multicolumn{1}{c|}{\textbf{Revision Items}} & \textbf{Requests} \\ \hline
\textbf{1}  & Clarify the contribution and goal in Section~\ref{sec:intro} and Section~\ref{sec:preliminary}.  & R1.O1 \\ \hline
\textbf{2}  & Further discuss the selection of document parsing tools.  & R1.O2 \\ \hline
\textbf{3}  & Add important related works like LayoutLMv3 and DocFormer.  & R1.O3 \\ \hline
\textbf{4}  & Add experiments of LayoutLMv3 and ablation studies.  & R1.O4 \\ \hline
\textbf{5}  & Add comparison and experiments on MP-DocVQA and M3DocVQA. & R1.O5 \\ \hline
\end{tabular}
}
\vspace{-.25cm}
\end{table}
\fi

\begin{shaded*}
\noindent
\hypertarget{R1.O1}{\textbf{R1.O1.}} The paper mixes goals across document parsing, structural modeling, and QA. It is not always clear which part constitutes the core scientific contribution.
\end{shaded*}

\noindent \textbf{Response:}
We thank the reviewer for the insightful feedback. Our work centers on structural modeling and QA, as the reviewer correctly pointed out. The document parsing is handled using existing OCR techniques (see \hyperlink{R1.O2}{R1.O2}) and is not the focus of our work. We have carefully revised our paper in \lspref{refine_goals}. 
%\yeye{line 244 has only one sentence for R1.O1? should this sentence mention about ``we use existing OCR'', or should we add hyperlinks here pointing to somewhere else that mentions about OCR?} to better clarify this positioning.
%We have carefully clarified the scope and contribution of our work:

% \begin{sloppypar}
% \noindent $\bullet$ \textbf{(1) Introduction (Section~\ref{sec:intro}):} We have clarified that our core contribution lies in \textbf{structural modeling and question answering}. Document parsing (e.g., OCR) is treated as a \zxh{preprocessing} step and is not the focus of this work. % We have clarified that our contribution centers on structural modeling and QA, as you pointed out. For document parsing, we rely on existing OCR as it is not our focus.
% \end{sloppypar}

% \begin{R1Box}
% \lspref{main_contribution} In summary, our contribution centers on structural modeling document elements and question answering based on them. For document parsing that extracts the original document elements, we rely on existing OCR techniques, which are not the focus of this work. \zxh{move to sec2.2}
% \end{R1Box}

% \noindent $\bullet$ \textbf{(2) Preliminaries (Section~\ref{sec:preliminary}):} We have refined the problem definition to emphasize QA as the \zxh{final} objective, with document parsing and structural modeling serving as enabling stages.

%We have refined the problem definition of semi-structured document analysis to a more general one. Its ultimate objective is to obtain an answer through QA , with document parsing and structural modeling serving as preliminary steps that facilitate the QA process.

% \begin{R1Box}
% \lspref{refine_goals} 
% \xbr{Note that \oursys centers on structural modeling document elements (to get components $\{\bm{\mathit{CO_{1}}}, ..., \bm{\mathit{CO_{m}}}\}$ and tree structure) and question answering based on them (to get the final answer \(\mathcal{A}\)).
% For document parsing that extracts the original document elements $\{\bm{\mathit{e_{1}}}, ..., \bm{\mathit{e_{n}}}\}$ from the document \(\mathcal{D}\), we rely on existing OCR techniques, which are not the focus of this work.}

% %To achieve this objective, we will first leverage existing document parsing tools to extract a series of elements $\{\bm{\mathit{e_{1}}}, ..., \bm{\mathit{e_{n}}}\}$ from the document \(\mathcal{D}\). Building upon this foundation, we will proceed with our design, encompassing both structural modeling (to get components $\{\bm{\mathit{CO_{1}}}, ..., \bm{\mathit{CO_{m}}}\}$ and tree structure) and question answering (to get the final answer \(\mathcal{A}\)). \zxh{-- rewrite: add note to clarify the goal}
% \end{R1Box}



\begin{shaded*}
\noindent
\hypertarget{R1.O2}{\textbf{R1.O2.}} The method relies on OCR text and bounding boxes, while other signals typically used by other approaches could help (e.g., native PDF structures, typographic cues)
\end{shaded*}


\noindent \textbf{Response:} This is an excellent observation. Our use of OCR was a deliberate design choice, as it provides a generalizable solution that applies uniformly across diverse real-world documents, including screenshots and scanned PDFs where native PDF structures are unavailable. We found that screenshots and scanned documents account for a significant portion of real documents -- for example, in benchmarks like DUDE, approximately 20\% of documents lack native PDF structures, rendering structure-based methods inapplicable, whereas our approach remains effective. We have clarified this design choice in \lspref{ocr_use}.

%This choice enables uniform preprocessing without assuming access to native PDF sources.


We would like to also clarify that \oursys does still leverage some typographic cues (e.g., font size and indentation) extracted via OCR and MLLM, for holistic layout and hierarchy understanding, while incorporating additional typographic cues remains part of our future work (\lspref{native_use}).

% \yeye{better to remove future work, it can be interpreted as we have not addressed it fully}
%As suggested by the reviewer, incorporating native PDF structures and typographic cues as auxiliary signals is a valuable enhancement, which we intend to explore as future work in \lspref{native_use}. 
% \end{sloppypar}

%  \xbr{utilized by OCR for element type identification and by hierarchy detection

%\zxh{derived from OCR outputs and MLLMs}

%While  can enhance structural modeling, they are often unavailable without native PDF support. 
% We acknowledge the potential of incorporating such signals when available and plan to explore this in future work.

\iffalse

% This is a great observation. We emphasize that our choice to use OCR was deliberate: it offers a generalizable approach that applies uniformly to the diverse real documents, including screenshots and scanned PDFs, where native PDF structures are not available and 

Besides, typographic cues (e.g., font and indentation) help identify document elements and hierarchies, but they can not be derived directly without native PDF structure. Instead, in our process, the OCR for document parsing and MLLM for hierarchy detection indirectly utilize these typographic cues presented in a visual manner.


The experimental analysis in Section~\ref{sec:sec:doc-preprocess} shows many documents do not involve native PDF structures (e.g., 20\% documents in DUDE~\cite{van2023document}, 10\% documents in ours) and directly parsed typographic cues like font name and size. But these signals can potentially benefit document modeling (e.g., verify OCR text and document hierarchy) if existing, which we will take as a future work.

% \noindent $\bullet$ \textbf{Document Preprocessing (Section~\ref{sec:sec:doc-preprocess}):} We have discussed and tested other document information extraction tools in Section~\ref{sec:sec:doc-preprocess}. 



\end{sloppypar}

\begin{R1Box}
\fnpage{ocr_use} 
Here we adopt OCR-based document parsing tool (e.g., PaddleOCR~\cite{cui2025paddleocr30technicalreport}), which can process documents in various formats, such as both digital documents and raster-based documents (such as screenshots and scanned PDFs). Other tools like pymupdf~\cite{pymupdf} and pdfplumber~\cite{pdfplumber} for native PDF parsing have their limitations, e.g., failing to parse 20\% documents in DUDE~\cite{van2023document}, 10\% documents in our newly created dataset without native PDF structures.

%Here we adopt OCR cause it can easily parse documents of various formats, such as screenshots and scanned PDFs which existing native PDF tools~\cite{pymupdf,van2023document} fails to handle.

%Here we choose OCR as the document-parsing tool, as it is a more versatile tool that can process both digital documents and raster-based documents (such as screenshots and scanned PDFs). We conduct an experiment to parse document using \zxh{pymupdf~\cite{pymupdf} and pdfplumber~\cite{pdfplumber}}, but they fail to parse some documents without native PDF structures. They are , and all PDFs of other two datasets~\cite{cho2024m3docrag, tito2023hierarchical} that are synthesized from our downloaded page images. \zxh{unclear}
\end{R1Box}

\begin{R1Box}
\lspref{native_use}
In the future, we will focus on further improving this system. In the preprocessing module, in addition to general parsing with OCR, we will incorporate native PDF structures and typographic cues for digital documents. For example, they provide important signals to help correct the OCR text (by text layer), element types and document hierarchy (by PDF tags / font name and size). In the construction module, the tree structure for one document can be naturally expanded to a forest for multiple documents. In the tree-based analysis module, we will explore more flexible retrieval methods (e.g., backtracking and skipping), to achieve enhanced retrieval performance
\end{R1Box}
\fi



\begin{shaded*}

\noindent
\hypertarget{R1.O3}{\textbf{R1.O3.}} Related work misses important contributions such as LayoutLMv3, DocFormer.
\end{shaded*}

% the model scale further limits its ability to handle context in long

\noindent \textbf{Response:} We appreciate the suggestion and have carefully added related works~\cite{huang2022layoutlmv3,appalaraju2021docformer} in \lspref{more_work1} and \lspref{more_work2} in response. Briefly, while both DocFormer~\cite{appalaraju2021docformer} and LayoutLMv3~\cite{huang2022layoutlmv3} can model input page-level images and OCR-extracted text, they mainly capture local relationships among document elements and lack holistic modeling of higher-level document structures, such as cross-block hierarchies and inter-section organization. Moreover, their constrained model capacity and limited maximum sequence length (e.g., 512 tokens in LayoutLMv3) hinder effective processing of long or multi-page documents.  We have also added experimental comparisons here, which we will discuss below. %which restricts their effectiveness in complex semi-structured document analysis tasks.


%We appreciate the suggestion. First, we have added these related works into Section~\ref{sec:intro} and Section~\ref{subsec:relatedwork}. While both LayoutLMv3 and DocFormer are capable of encoding textual and visual information, they primarily captures sequential relationships among document elements and struggles to model higher-level document structures. In addition, they are designed to support page-level input up to a limited length (e.g., within {maximum sequence length 512 for text tokenization}), which restrict their straightforward extension to multi-page document processing.

% \noindent $\bullet$ \textbf{(1) Introduction (Section~\ref{sec:intro}):}
% We have added LayoutLMv3 and DocFormer in the introduced related works.

% \begin{R1Box}
% \lspref{more_work1} (4) End-to-End models including pre-trained models and Multimodal Large Language Models (MLLMs), such as LayoutLMv3~\cite{huang2022layoutlmv3}, DocFormer~\cite{appalaraju2021docformer} ...
% \end{R1Box}

% \noindent $\bullet$ \textbf{(2) Limitations of Existing Methods (Section~\ref{subsec:relatedwork}):}
% We have carefully discussed the limitations of LayoutLMv3 based on experimental results.


% Second, pilot study (Section~\ref{subsec:relatedwork}) and experiments (Section ~\ref{sec:experiments}) show LayoutLMv3 and DocFormer fall far short of MoDora. On DUDE, for instance, LayoutLMv3 reaches 25.06 AIC-Acc and 23.43 ACNLS -- higher than models like UDOP, yet still far below MoDora's 83.70 and 77.24. A similar gap appears on MMDA, where LayoutLMv3 obtains 17.37 (AIC-Acc) and 13.96 (ACNLS), which are significantly lower than MoDora's 73.33 and 55.23. \xbr{This comes from their limitations in complex document structure understanding and multi-page input adaptation.}

% \begin{R1Box}
% \lspref{more_work2} ... DocFormer, LayoutLMv3, and UDOP input page-level document information (e.g., page images, OCR-parsed text, bounding boxes) directly into pretrained transformer models. They primarily capture local and sequential relationships among document elements and lack explicit modeling of higher-level document structures, such as cross-block hierarchies and inter-section organization. Moreover, their limited model scale and maximum sequence length (e.g., 512 text tokens in LayoutLMv3) make it difficult to process lengthy or multi-page documents, which restricts their effectiveness on complex semi-structured document analysis tasks.
% \end{R1Box}


\begin{shaded*}
\noindent
\hypertarget{R1.O4}{\textbf{R1.O4.}} Experimental evaluation does not fully support the claims: comparisons are primarily against simple baselines rather than other similar models (see O3); the ablation study does not isolate the impact of each major component (component reconstruction, hierarchical representation, retrieval strategy); the improvements shown are limited.
\end{shaded*}


%Thank you for your valuable suggestions. First, we have added the comparison with LayoutLMv3 (\xbr{DocFormer is a much earlier work and the fine-tuned version for question answering is not publicly available}), which \xbr{obtains an AIC-Acc of only 25.06 versus \oursys 's 83.70 on dataset DUDE}. Additionally, experimental analysis with most recent works like ZenDB and DocAgent also verifies our superiority (\xbr{with 15\% accuracy improvement}).
\begin{sloppypar}
\noindent \textbf{Response:} 
We agree that these suggestions can substantially strengthen our experiments, and we have added the corresponding results to the revised paper as suggested.
\end{sloppypar}

We have added results using LayoutLMv3 in both the pilot study ({\emph{\textbf{Figure~\ref{fig:precompare}}}}) and the main experiments ({\emph{\textbf{Figure~\ref{fig:trend}}}}, {\emph{\textbf{Table~\ref{tab:type}}}} and \lspref{main_discussion}). On DUDE, LayoutLMv3 reaches 25.06 AIC-Acc and 23.43 ACNLS -- higher than UDOP, yet still far below MoDora's 83.70 and 77.24. A significant gap also exists on MMDA, where LayoutLMv3 obtains 17.37 (AIC-Acc) and 13.96 (ACNLS), significantly lower than MoDora's 73.33 and 55.23. (We omit DocFormer as it is an older technique that lacks a public QA-tuned version for us to run, and LayoutLMv3 has also been shown to outperform Docformer in a variety of document processing tasks~\cite{huang2022layoutlmv3}). 

%\yeye{can we find evidence from other papers, that DocFormer performs worse than LayoutLMv3, in any tasks that are not limited to non-QA tests? We can cite such results here to say why we did not compare DocFormer b/c it is old and weaker than LayoutLMv3.}

We have added detailed ablation results
for the suggested analysis in \lspref{re_ablation} and  {\emph{\textbf{Table~\ref{tab:ablation}}}}. We show that: 
%for the three variants of our system: (i) \oursys w/o tree structure, (ii) \oursys w/o forward retrieval, and (iii) \oursys with all three components removed, i.e., TextRAG, (see \lspref{re_ablation} and  {\emph{\textbf{Table~\ref{tab:ablation}}}}): 

%We have added results of three variants (i.e., \oursys w/o tree structure, w/o forward retrieval, w/o all three components (TextRAG)) in ablation study (\lspref{re_ablation} and  {\emph{\textbf{Table~\ref{tab:ablation}}}}): 


% and have the following findings \xbr{(TextRAG)}

\noindent(1) Removing the ``hierarchical representation'' component (corresponding to ``w/o tree structure'' in  {\emph{\textbf{Table~\ref{tab:ablation}}}}) causes a significant drop in AIC-Acc on MMDA -- from 73.33 to 57.84, highlighting the importance of tree structure for modeling document hierarchies (e.g., nested chapters), to enable hierarchy-aware evidence localization (e.g., CaseID 4, 5 in Figure~\ref{case_study}). % in Figure~\ref{fig:multilayout}

% principled retrieval paths, especially for questions that are strongly tied to the document’s hierarchy

\noindent(2) Removing the ``retrieval strategy'' (corresponding to ``w/o {Forward Search}'' in {\emph{\textbf{Table~\ref{tab:ablation}}}}) also leads to a sizable drop in accuracy (up to 5.30 points), because retrieval guided by metadata help to reliably navigates to locate relevant document information. In contrast, embedding-based search over trees is more prone to errors.

%can steadily select appropriate branches to explore relevant  document information, whereas embedding search on tree, used as a fallback, is less reliable. 


\noindent(3) Removing ``component reconstruction'' is not entirely straightforward in our system, as it is an essential building block in \oursys (without which we can not build a document tree on raw elements). Nevertheless, we added a variant that removes component reconstruction as well as subsequent steps that depend on it (which is similar to TextRAG). This leads to the method  denoted as ``w/o component reconstruction'' in {\emph{\textbf{Table~\ref{tab:ablation}}}}, which performs more than 27 points worse than \oursys. 

%While the component-reconstruction module cannot be ablated independently, as it serves as the foundation for hierarchical representation and retrieval

% \noindent $\bullet$ \textbf{Ablation Study (Section~\ref{subsec:ablation}):}
% We have refined the description of the retrieval strategy ablation that replace LLM forward search by embedding search, as well as included the discussion of newly added ablation of tree structure in Section~\ref{subsec:ablation}.

% \begin{R1Box}
% \lspref{re_ablation} We \xbr{remove} the LLM forward search, meaning that LLM is no longer used to choose nodes based on their titles and metadata. Instead, embedding search and backward verification are performed on the tree. Tree nodes continue to serve as chunk boundaries, node paths are still used to provide context, and the answering model maintains the chance to refer to the entire CCTree in cases where retrieval fails.

% \lspref{hi_ablation} We isolate the impact of hierarchical representation via conducting question answering based on the flattened components with the same retrieval strategies. Without the assistance of tree structure, the AIC-Acc decreases greatly by -15.33\% and -15.49\% on DUDE and \oursys respectively. This demonstrates the utility of our structural modeling of CCTree.
% \end{R1Box}

% \begin{R1Box}
% \lspref{textrag_ablation} 
% (5) Retrieval-Augmented Generation (RAG) methods~\cite{cho2024m3docrag, chen2024sv, hegde2023analyzing} retrieve document chunks at coarse granularity and lack structural alignment, which result in missing or misaligned evidence during multi-element reasoning.
% TextRAG retrieves relevant semantic pieces from chunks of OCR output~\cite{hegde2023analyzing}, while SV-RAG~\cite{chen2024sv} and M3DocRAG~\cite{cho2024m3docrag} retrieve relevant page images.
% \end{R1Box}


%First, we have added new baselines (including LayoutLMv3, DocFormer, \zxh{xxx}), which fall far short of \oursys (see \zxh{Rx.Oy, ...}). %such as LayoutLMv3, which still fall far short of \oursys. On DUDE, for instance, LayoutLMv3 reaches 25.06 AIC-Acc and 23.43 ACNLS – higher than models like UDOP, yet still far below \oursys's 83.70 and 77.24. A similar gap appears on MMDA, where LayoutLMv3 obtains 17.37 (AIC-Acc) and 13.96 (ACNLS), which are significantly lower than \oursys's 73.33 and 55.23. 

% \noindent $\bullet$ \textbf{Experiments (Section~\ref{sec:experiments}):} We have added the detailed experimental results of newly added baselines including LayoutLMv3.

% \begin{R1Box}
% \lspref{type_discussion} As shown in Table~\ref{tab:type}, \oursys achieves the best performance across all four question types defined in Section~\ref{subsec:questiontype}, demonstrating the effectiveness in capturing structural, textual, hybrid, and spatial information for document understanding...
% \end{R1Box}

%\noindent\ding{183} Second, as suggested, w



\begin{shaded*}
\noindent
\hypertarget{R1.O5}{\textbf{R1.O5.}} MMDA is relatively small, and its construction may introduce an inherent selection bias: documents are chosen based on ViT embeddings and on the ED/LD metrics, which explicitly favor files containing a high number of element types and multiple independent components per page. As a result, the dataset is, by design, skewed toward structurally complex and visually heterogeneous documents. It is a useful stress-test, but it does not reflect a real-world document distribution. Authors could extend their evaluation also on other benchmark, such as the cited MP-DocVQA and M3DocVQA to better demonstrate the generality of the approach.
\end{shaded*}

\noindent \textbf{Response:} We thank the reviewer for the insightful comment. To demonstrate the generality of our approach, we have added the two suggested benchmarks, MP-DocVQA and M3DocVQA, and tested all methods on these benchmarks, with our  results presented in {\emph{\textbf{Figure~\ref{fig:trend}}}} and \lspref{main_discussion}. On MP-DocVQA, \oursys outperforms GPT-5 by 13 percentage points in accuracy, and achieves a 12-point improvement on M3DocVQA. These results show that \oursys is effective not only on \ourbench, but also on simpler benchmarks such as MP-DocVQA and M3DocVQA, highlighting its strong generalizability. % (see \hyperlink{R1.O4}{R1.O4}).

The reviewer is correct that MMDA is intentionally constructed to capture structurally complex layouts often encountered in real-world scenarios (e.g., business reports, financial tables). While the size of the benchmark (537) is comparable to prior benchmarks like MP-DocVQA (959)~\cite{tito2023hierarchical},  it does exhibits higher layout diversity and complexity. As shown in {\emph{\textbf{Table~\ref{tab:datasets}}}} of our revised paper, MMDA has more nodes per tree on average (49.2 vs. 38.3 in M3DocVQA), and a lower ED score (0.264 vs. 0.305 in MP-DocVQA, with lower ED indicating richer element variation). We have added {\emph{\textbf{Figure~\ref{fig:cluster1}}}} to visualize document layout distributions that compare \ourbench with MP-DocVQA and M3DocVQA, as well as corresponding analysis in \lspref{dataset_ana} and \lspref{cluster}. 

%Thank reviewer for the insightful comment. The reviewer is correct that MMDA is explicitly designed to capture the complex document layouts frequently seen in real-world applications (e.g., business reports, financial tables). The test dataset's size (537) is comparable to MP-DocVQA (959)~\cite{tito2023hierarchical} and shows competitive layout diversity. For instance, as shown in {\emph{\textbf{Table~\ref{tab:datasets}}}}, MMDA has 49.2 nodes per tree vs. 38.3 in M3DocVQA, and achieves lower ED (0.264 vs. 0.305 in MP-DocVQA), indicating greater diversity in element types. %Here ED denotes the normalized standard variance in the counts of different element types and lower ED indicates higher element diversity. We have revised {\emph{\textbf{Figure~\ref{fig:cluster1}}}} to add the document layout distributions of MP-DocVQA and M3DocVQA and added discussions in \lspref{cluster}.


% When other approaches are still disturbed by multi-page and cross-modal contents in analysis of these two benchmarks (e.g., combining text and figures in wiki for inference, extracting content from scanned forms), \oursys uniformly construct them into a CCTree and derive the answer via its modules
%\oursys outperforms GPT-5 by 13\% on MP-DocVQA and by 12\% on M3DocVQA, confirming its effectiveness on benchmarks with relatively simpler structures and questions than \ourbench.



%We have updated the distribution of pages from documents of MP-DocVQA and M3DocVQA in the embedding space in {\emph{\textbf{Figure~\ref{fig:cluster1}}}}, and discussed the distinct clusters brought by wiki pages in M3DocVQA and scanned pages in M3DocVQA (see \lspref{cluster}).


%\yeye{need to briefly say what LD is here. Also it is not clear what the point is here -- are we trying to say that we have ``lower'' diversity than M3DocVQA (if so why is it a good thing for us, in response to the comment?)}

% its size is comparable to other benchmarks like MP-DocVQA (which has 959).  We agree that MMDA emphasizes complex layouts by design, serving as a challenging stress-test. However, its construction is grounded in practical needs: the 537 documents were carefully sampled from one million real-world files (e.g., financial, business, academic), ensuring representativeness.

%The reviewer is correct that MMDA is explicitly designed to capture the complex document layouts frequently seen in real-world applications (e.g., business reports, financial tables). The test dataset owns 537 documents, carefully selected from {one million diverse documents} to ensure strong representativeness, and its size is comparable to other benchmarks like MP-DocVQA (which has 959). As shown in Table~\ref{tab:datasets}, \ourbench achieves lower LD (0.264 compared to 0.305 of MP-DocVQA), higher LD (1.85 compared to 1.35 of DUDE) and more tree nodes (49.2 compared to 38.3 of M3DocVQA). These optimal statistics indicate its richer document element types, complexity of layout distribution, and sufficiency of content. \ourbench has fewer average CCTree levels than M3DocVQA, which is partly attributable to the fact that M3DocVQA consists of Wikipedia documents, which inherently possess more hierarchical title levels, whereas \ourbench also encompasses some document types with fewer heading levels.


%\noindent \ding{183} Second, although we have evaluated MoDora on DUDE (another benchmark with simpler documents), we also include experiments using MP-DocVQA / M3DocVQA in the revised paper, as suggested.

% \noindent $\bullet$ \textbf{(1) Micro Benchmark Preparation(Section~\ref{ssec:bench}):} We have discussed the differences between datasets and compared their statistics.

% \begin{R1Box}
% \lspref{dataset_ana} Existing datasets cannot well reflect the complexity of typical semi-structured document analysis tasks~\cite{tito2023hierarchical,cho2024m3docrag,van2023document}. The documents in MP-DocVQA~\cite{tito2023hierarchical} and DUDE~\cite{van2023document} exhibit limitations in content sufficiency, element richness and structural complexity. While M3DocVQA~\cite{cho2024m3docrag} are more challenging in these aspects, its documents are sourced from Wikipedia, lacking representativeness of other types of complex documents. Thus, in this section we introduce a new benchmark \oursys.
% \end{R1Box}



%open-ended document questions by leveraging structured document modeling through CCTree and fine-grained retrieval guided by layout and semantic cues (see \hyperlink{R1.O4}{R1.O4}).

%It verifies that \oursys can better perform for other general document questions via effective and generalizable designs, such as tree-structured modeling and retrieval strategies (see \hyperlink{R1.O4}{R1.O4}).

%They also benefit from \oursys's local-alignment aggregation to integrate elements, tree construction to organize various components, and the retrieval process that leverages both semantic and locational cues to optimize the recall and precision.

% \begin{R1Box}
% \lspref{dataset_cmp} Besides, we compute various statistics for the four datasets, including the previously defined ED and LD, as well as the average number of nodes, leaves and levels of the CCTree constructed based on their documents. As shown in Table~\ref{tab:datasets}, \ourbench achieves lower ED (0.264 compared to 0.305 of MP-DocVQA), higher LD (1.85 compared to 1.35 of DUDE) and more tree nodes (49.2 compared to 38.3 of M3DocVQA). These optimal statistics indicate its richer document element types, complexity of layout distribution, and sufficiency of content. \ourbench has fewer average CCTree levels than M3DocVQA, which is partly attributable to the fact that M3DocVQA consists of Wikipedia documents, which inherently possess more hierarchical title levels, whereas \ourbench also encompasses some document types with fewer heading levels.
% \end{R1Box}

%\noindent $\bullet$ \textbf{(2) Experiments (Section~\ref{sec:experiments}):} We have added the experimental results of these datasets.

%on MP-DocVQA, \oursys achieves 13\% accuracy compared to GPT-5, and on M3DocVQA, the leading is 12\%. They also benefit from \oursys's local-alignment aggregation to integrate elements, tree construction to organize various components, and the retrieval process that leverages both semantic and locational cues to optimize the recall and precision. 
%\zxh{Second, experimental analysis on MP-DocVQA and M3DocVQA shows that MoDora consistently outperforms all baselines. On MP-DocVQA, MoDora achieves 78.5\% AIC-Acc, which is 13\% higher than GPT-5 (65.5\%). On M3DocVQA, MoDora leads by 12\%, achieving 72.3\% AIC-Acc compared to 60.3\% for the best baseline. These results further validate the effectiveness of our tree-based approach on diverse benchmarks.}

% \begin{R1Box}
% xxx
% \end{R1Box}

\section*{Response to Reviewer \#2 \textcolor{orange}{(Orange)}}

\iffalse
\begin{table}[!h]
\vspace{-.5cm}
\caption{Revision Summary for Reviewer \#2.}
\vspace{-.35cm}
\label{tab:reviewer2}
\resizebox{.95\linewidth}{!}{
\begin{tabular}{c|l|c}
\hline
\textbf{ID} & \multicolumn{1}{c|}{\textbf{Revision Items}} & \textbf{Requests} \\ \hline
\textbf{1}  & Add comparison and experiments of referred related works. & R2.O1 \\ \hline
\textbf{2}  & Clarify MoDora's ability to handle complex queries & R2.O2. \\
\textbf{3}  & Test MoDora on ZenDB's dataset and metrics.  & R2.O2 \\ \hline
\textbf{4}  & Discuss the concerns of metric designs and relevant experiment results.  & R2.O3 \\
\textbf{5}  & Clarify parameter settings for experiments in Section~\ref{subsec:setup}. & R2.O3 \\
\textbf{6}  & Clarify the description and analysis of the ablation study in Section~\ref{subsec:ablation}. & R2.O3 \\ 
\textbf{7}  & Explain the usage scenarios of such questions in Section~\ref{subsec:questiontype}. & R2.O3 \\ \hline
\end{tabular}
}
\vspace{-.35cm}
\end{table}
\fi

\begin{shaded*}
\noindent
\hypertarget{R2.O1-(1)}{\textbf{R2.O1-(1).}} The paper has limited novelty, with tree-based construction and traversal similar to SHT [13].
%The paper has limited novelty. The main technical contribution is a tree-based retrieval method which is very similar to the SHT of [13], which minor differences such as additional nodes for non-text data, and both construction and traversal of the tree is also very similar to SHTs. 
%Other pieces of the solution, such as backward validation or location-based retrieval are also common and straightforward. There are also many other papers that incorporate similar ideas [a, b, c]

% [a] https://aclanthology.org/2025.emnlp-main.893.pdf

% [b] https://aclanthology.org/2025.naacl-industry.45.pdf

% [c] https://aclanthology.org/2024.emnlp-industry.13.pdf

\end{shaded*}

\noindent \textbf{Response:}  We agree with the reviewer that SHT [13] is indeed seminal in document processing (which we have emphasized more in our revised paper, in \lspref{more_work3}). We note however that tree-based method is a widely used in semi-structured documents (e.g., also adopted in [a–c] cited by the reviewer), and therefore does not on its own limit the novelty of our approach.

 
 We want to highlight that \textit{MoDora is designed from the ground up in ways that fundamentally distinguish it from SHT}. 
 As discussed in \lspref{more_work5}, at a conceptual level, MoDora natively supports multi-modal documents and performs holistic modeling over non-textual elements such as tables, charts, and images, enabling integrated multi-modal reasoning. In contrast, SHT operates on text only and can fail to handle over 60\% of hybrid analysis questions in \ourbench that involves non-textual data (see \emph{\textbf{Table~\ref{tab:type}}}). 
 Furthermore, MoDora generalizes well to diverse document formats, including screenshots and scanned PDFs, whereas SHT relies on the availability of native PDF structures, which are often missing in real world documents (e.g., account for over 20\% of cases in DUDE).
 
Beyond these conceptual distinctions, \oursys incorporates several key algorithmic innovations that further set it apart (see \lspref{main_contribution}), including:
\begin{enumerate}[leftmargin=*, itemsep=0pt, labelindent=0pt,
  itemindent=0pt]
\item \underline{Document Layout}: MoDora holistically combines local layout, MLLM-based hierarchy detection, and main-body/supplement separation (Sections~\ref{sec:sec:doc-preprocess} and ~\ref{sec:sec:cctree}) to construct accurate CCTree, whereas SHT's visual clustering can often be confused by colorful headers/titles/captions, yielding 23\% suboptimal performance in hierarchies (see \emph{\textbf{Table~\ref{tab:type}}}).

\item \underline{Summarization}: MoDora develops an information attenuation formulation (Section~\ref{sec:sec:cctree}), to preserve essential content while minimizing redundancy. 

\item \underline{Data Search}: MoDora parses queries to extract both locational and semantic cues, and then integrates search with verification to improve answer quality (see Section~\ref{sec:sec:doc-analysis}). 
\end{enumerate}

Precisely because of these conceptual distinctions and algorithmic advances, MoDora delivers stronger empirical results, like we reported in the original paper which compares \oursys with SHT on the DUDE and MMDA benchmarks. In order to conclusively show the performance benefit of MoDora over SHT, during revision, we have significantly expanded our experimental evaluation, by adding: 
\begin{enumerate}[leftmargin=*, itemsep=0pt, labelindent=0pt,  itemindent=0pt]
\item Comparisons of MoDora and SHT, using the same three benchmarks (Civic, Qasper, Contract), and metrics (precision, recall, F1) from the SHT paper, which we show in \emph{\textbf{Table~\ref{tab:sht}}} and \lspref{sht_test} of the revised paper. \oursys consistently outperforms SHT across all the three new datasets -- on the Civic dataset, for example, MoDora achieves 77.3 accuracy, 89.4 precision, and 71.1 recall, substantially better than SHT at 71.8, 81.5, and 42.7, respectively.  %Similarly, For dataset qasper, \oursys has a higher F1 score (35.6 vs. 31.8). And for dataset contract, \oursys has higher accuracy (90.6 vs. 85.7).
\item  Comparisons of MoDora and SHT, using two new VQA benchmarks, MP-DocVQA~\cite{tito2023hierarchical} and and M3DocVQA~\cite{cho2024m3docrag}, like shown in \emph{\textbf{Figure~\ref{fig:trend}}}} and \lspref{main_discussion}. On MP-DocVQA, \oursys achieves 19 percentage point higher accuracy compared to SHT, and 58 point better accuracy on M3DocVQA, which further validates the advantage of \oursys over SHT.
\end{enumerate}

We believe all of these are valuable additions to our paper, as they now help to conclusively demonstrate the robust generalizability of \oursys across seven benchmarks (Civic, Qasper, Contract, DUDE, MMDA, M3DocVQA, and MP-DocVQA), using diverse evaluation metrics (precision, recall, f1, ACNLS, AIC-Acc), and we thank the reviewer for the suggestion.



\begin{shaded*}
\noindent
\hypertarget{R2.O1-(2)}{\textbf{R2.O1-(2).}} 
 Other pieces of the solution, such as backward validation or location-based retrieval are also common and straightforward, similar to [a, b, c]

% [a] https://aclanthology.org/2025.emnlp-main.893.pdf

% [b] https://aclanthology.org/2025.naacl-industry.45.pdf

% [c] https://aclanthology.org/2024.emnlp-industry.13.pdf

\end{shaded*}
MoDora differs fundamentally from the works cited in [a, b, c], which we discuss in \lspref{more_work3} and \lspref{more_work4} of the revised paper. In terms of backward validation, MoDora performs fine-grained node-level verification, explicitly checking the underlying document evidence for each retrieved candidate to filter out false positives introduced by summary-based selection. In contrast, the reviewer agent in~[a] validates the reasoning trajectory and final answer to decide whether further analysis is needed, rather than validating document evidence itself. For location-based retrieval, MoDora supports in-page region-level alignment through orientation–grid mapping, whereas prior works~[a, b, c] retrieve at the coarse page level at most, which limits precision for densely structured layouts.

In order to convincingly show these key differences, we have now included a direct experimental comparison  with DocAgent~[a] which is one of the strongest method in this group. Like we show in  \emph{\textbf{Figure~\ref{fig:precompare}}}, \emph{\textbf{Figure~\ref{fig:trend}}}, \emph{\textbf{Table~\ref{tab:type}}} and \lspref{main_discussion} of the revised paper, DocAgent scores 57.09 AIC-Acc and 37.10 ACNLS on \ourbench, which are about 15 percentage points lower than the results achieved by \oursys, underlying the key differences between \oursys and methods like [a].

%We have added relevant discussions and results in \lspref{more_work3}, \lspref{more_work4}, \lspref{type_discussion}, \emph{\textbf{Figure~\ref{fig:precompare}}}, \emph{\textbf{Figure~\ref{fig:trend}}} and {\emph{\textbf{Table~\ref{tab:type}}}}.

%We thank the reviewer for the valuable comment. We agree that SHT [13] is a seminal work in document processing (which we have emphasized more in Section~\ref{sec:intro} and {Section~\ref{subsec:relatedwork}}). However, we want to highlight that \bfit{MoDora is designed from the ground up with capabilities fundamentally different from SHT}:

%\noindent \ding{182} \textbf{Multi-Modal Support.} 

%\noindent \ding{183} \textbf{Format-Agnostic.} 

%\noindent \ding{184} \textbf{End-to-End QA System.} 

% \noindent\ding{182} Multi-Modal Support: MoDora supports multi-modal documents that integrate non-textual elements such as tables, charts, and images (whereas SHT operates on plain text and therefore misses over 20\% of cases in MMDA).

% \noindent\ding{183} Broader Applicability: MoDora is applicable to a broad range of documents, including screenshots and scanned PDFs (whereas SHT relies on the ones with native PDF structures as reported in its paper).

%We want to highlight that MoDora is designed from the ground up with capabilities fundamentally different from SHT: MoDora supports multi-modal documents that integrates non-textual elements such as tables, charts, and images (whereas SHT operates on plain text and therefore misses over 20\% of cases in MMDA). Additionally, MoDora is applicable to a broad range of documents, including screenshots and scanned PDFs (whereas SHT relies on the ones with native PDF structures as reported in its paper).


% \noindent\ding{184} Algorithmic Advances: These differences come in addition to several key algorithmic advances, such as (i) [Document Layout]: MoDora holistically combines local layout, MLLM-based hierarchy detection, and main-body/supplement separation (Sections 4 and 5) to construct accurate CCTree, whereas SHT's visual clustering is often confused by colorful headers/titles/captions, yielding 30\% suboptimal hierarchies. (ii) [Summarization]: MoDora follows an information attenuation formula (see Section 5), to preserve essential content while minimizing redundancy. (iii) [Data Search]: MoDora parses a query to get locational and semantic cues, and then performs a combination of search and verification steps to improve quality (see Section 6).

\iffalse

These differences come in addition to several key algorithmic advances, such as
(i) [Document Layout]: MoDora holistically combines local layout, MLLM-based hierarchy detection, and main-body/supplement separation (Sections \ref{sec:sec:doc-preprocess} and \ref{sec:sec:cctree}) to construct accurate CCTree, whereas SHT's visual clustering is often confused by colorful headers/titles/captions, yielding ~30\% suboptimal hierarchies.
(ii) [Summarization]: % While SHT directly extracts summaries from plain text, 
\oursys follows an information attenuation formula (see Section~\ref{sec:sec:cctree}), to preserve essential content while minimizing redundancy. (iii) [Data Search]: \oursys  parses a  query to get locational and semantic cues, and then performs a combination of search and verification steps to improve quality (see Section~\ref{sec:sec:doc-analysis}). %In contrast, the retrieval in SHT often leads to false positives due to semantic drift (e.g., returning bitcoin definitions when retrieving the release time of bitcoin related policies).
\fi

%We thank reviewer for the valuable comment. We agree with the reviewer that SHT [13] is clearly a seminal work in document processing (which we have emphasized more in Section~\ref{sec:intro} and {Section~\ref{subsec:relatedwork}}). However, we should note that tree-based approach is a natural and common choice for processing semi-structured documents (e.g., also adopted in [a–c] cited by the reviewer), and therefore does not on its own limit the novelty of our approach.

% etrieval is widely used in semi-structured documents (e.g., also adopted in [a–c] cited by the reviewer), and therefore does not on its own limit the novelty of our approach. 



% These differences come in addition to several key algorithmic advances, such as
% (i) [Document Layout]: MoDora holistically combines local layout, MLLM-based hierarchy detection, and main-body/supplement separation (Sections \ref{sec:sec:doc-preprocess} and \ref{sec:sec:cctree}) to construct accurate CCTree, whereas SHT's visual clustering is often confused by colorful headers/titles/captions, yielding ~30\% suboptimal hierarchies.
% (ii) [Summarization]: % While SHT directly extracts summaries from plain text, 
% \oursys follows an information attenuation formula (see Section~\ref{sec:sec:cctree}), to preserve essential content while minimizing redundancy. (iii) [Data Search]: \oursys  parses a  query to get locational and semantic cues, and then performs a combination of search and verification steps to improve quality (see Section~\ref{sec:sec:doc-analysis}).

%\noindent\ding{182} First, we highlight that MoDora is designed from the ground up with capabilities fundamentally different from SHT: MoDora supports multi-modal documents that integrates non-textual elements such as tables, charts, and images (whereas SHT operates on plain text and therefore misses over 20\% of cases in MMDA). Additionally, MoDora is applicable to a broad range of documents, including screenshots and scanned PDFs (whereas SHT relies on the ones with native PDF structures as reported in its paper).


% \noindent $\bullet$ \textbf{Introduction (Section~\ref{sec:intro}):}
% We have carefully refined the introduction of structure extraction methods in Section~\ref{sec:intro}, comparing the differences between SHT and other three works you mentioned, as well as discussing their limitations in document modeling and analysis.


% \begin{R3Box}
% \lspref{more_work3}(2) Structure extraction methods like ZenDB~\cite{zendb} employ visual feature clustering and LLMs to extract the partial document structure SHT (e.g., distinguishing titles from body text), and raise a summarization mechanism to guide the search. Although SHT is good at \xbr{capturing the basic semantic hierarchy of titles and text}, it fails on many complex layouts, such as often misidentifying hierarchical levels and table regions, neither integrates the ability to process charts and images.
% In addition, works such as DocAgent~\cite{sun2025docagent}, SuperRAG~\cite{yang2025superrag}, and PDFTriage~\cite{saad2024pdftriage} also employ structural documents modeling. However, due to the document parsing methods and node definitions, they also fail to align textual data and bounding box locations of document elements at the tree/graph node level. \xbr{As a result, they exhibit limitations or require additional steps when processing non-digital documents or elements such as tables and charts.} %\zxh{Furthermore, their retrieval mechanisms also vary. For instance, agent interaction, vector search and intermediate languages.}
% \end{R3Box}

% Precisely because of these key differences, MoDora delivers stronger empirical results. In addition to what we report in the submitted paper, we have tested MoDora on the benchmarks and metrics used by SHT to further validate these gains – on Civic, for example, MoDora has accuracy 77.3, precision 89.4, and recall 71.1, substantially outperforming SHT at 71.8, 81.5, and 42.7, respectively (using its publicly released result with default parameters). Similarly, For dataset qasper, \oursys has higher f1 score (35.6) compared to SHT (31.8). And for dataset contract, \oursys has higher accuracy (90.6) compared to SHT (85.7).

% \oursys also differs in important ways from the works [a, b, c] cited in the review: (1) The backward validation in \oursys individually checks the data of each candidate node, excluding false positives resulting solely from summary-related selection. While the reviewer agent in [a] checks the analysis trajectory and primary answer to determine to take further analytical operations or to derive a final answer. (2) For locational-based retrieval, \oursys supports in-page-level location based retrieval by orientation-grid mapping. While [a, b, c] retrieve by whole pages at most. 

% We have added experiments comparing against the baselines [a] cited by the reviewer. The results show that DocAgent [a] achieves 37.10 ACNLS and 57.09 AIC-Acc on MMDA, which still falls behind MoDora by 15\%. We have updated Section~\ref{subsec:relatedwork} and Section~\ref{sec:experiments} with detailed comparisons.


% \begin{R3Box}
% \lspref{sht_test}
% We further test \oursys and compared with ZenDB's result on its datasets and metrics (available in ~\cite{sht}). As shown in Table~\ref{{tab:sht}}, \oursys also achieve better overall performance, showing its generalization to other datasets and metrics.
% \end{R3Box}

% \oursys also differs in important ways from the works [a, b, c] cited in the review: (1) The backward validation in \oursys individually checks the data of each candidate node, excluding false positives resulting solely from summary-related selection. While the reviewer agent in [a] checks the analysis trajectory and primary answer to determine to take further analytical operations or to derive a final answer. (2) For locational-based retrieval, \oursys supports in-page-level location based retrieval by orientation-grid mapping. While [a, b, c] retrieve by whole pages at most. 

% We have added experiments comparing against the baselines [a] cited by the reviewer. The results show that DocAgent [a] achieves 37.10 ACNLS and 57.09 AIC-Acc on MMDA, which still falls behind MoDora by 15\%. We have updated Section~\ref{subsec:relatedwork} and Section~\ref{sec:experiments} with detailed comparisons.

%We have added experiments comparing against all three baselines [a], [b], and [c] cited by the reviewer (see Section 8). The results show that DocAgent [a] achieves 37.10 ACNLS and 57.09 AIC-Acc on MMDA, which still falls behind MoDora by 15\%. \zxh{Similarly, [b] and [c] achieve [X.XX] and [Y.YY] AIC-Acc respectively, further confirming MoDora's superiority.} We have updated Section 8 with these detailed comparisons.

%We have added experiments comparing against the baselines [a] \zxh{what about [b], [c]?} (see Section~\ref{sec:experiments}), which has 37.10 ACNLS and 57.09 AIC-Acc on MMDA, and still falls behind \oursys by 15\%. 

% \begin{R3Box}
% \lspref{more_work4} 
% DocAgent~\cite{sun2025docagent} extracts document contents into a XML tree structure outline, which guides the agent to act and review based on predefined tools (e.g. search by keywords, page, section id, image id and table id). But the execution of actions and reviews is not closely integrated with the tree, and the model needs to understand the tree structure on its own when retrieving and reasoning, which makes it more prone to mistakes.

% \lspref{type_discussion} As shown in Table~\ref{tab:type}, \oursys achieves the best performance across all four question types defined in Section~\ref{subsec:questiontype}, demonstrating the effectiveness in capturing structural, textual, hybrid, and spatial information for document understanding...
% \end{R3Box}


\begin{shaded*}
\noindent
\hypertarget{R2.O2}{\textbf{R2.O2.}} Meanwhile, compared with [13], the paper only supports limited queries. It only focuses on look-up style questions. Other question types (e.g., aggregates of values, especially since there are tables in the documents) as well as more complex multi-hop questions documents with tables are not supported.
\end{shaded*}

\noindent \textbf{Response:} We would like to respectfully clarify that MoDora supports all query types handled by SHT [13], including aggregations and multi-hop questions, which we highlight more in \lspref{complex_query} of our revised paper. 

In order to show that MoDora can indeed handle the queries that SHT handles, we also added experiments in {\emph{\textbf{Table~\ref{tab:sht}}}} to test MoDora using the benchmarks used by SHT (see \hyperlink{R2.O1-(1)}{R2.O1-(1)}), which include diverse query types beyond look-up style questions. Our results show that \oursys can indeed handle diverse queries (e.g., {value aggregation or filtering queries like ``projects in status `design' and type `capital' ''}) from the SHT benchmark. In fact, \oursys produces results with substantially higher quality  (up to 28 percentage points higher using SHT's  datasets and evaluation metrics).

% Identify and list the names of all 


%quality when compared to the original results reported in the SHT paper on these benchmarks.

% \noindent\ding{182} First, we respectfully clarify that MoDora supports all query types handled by SHT [13], including aggregations and multi-hop questions. 

% \noindent $\bullet$ \textbf{Experiments (Section~\ref{sec:experiments}):} We have clarified \oursys's existed ability to handle complex queries and the possibility of further enhancement in Section~\ref{subsec:questiontype}.

% \begin{R3Box}
% \lspref{complex_query} 
% Note \oursys effectively handles questions of above types (see experiments in Section~\ref{subsec:overallperformance}), and can also process more complex multi-step questions (e.g. values aggregation and conditional query), which can be regarded as a composite of the above-mentioned basic types. This achievement comes from the multi channel retrieval on the tree and comprehensive analysis capability of \llms (see cases in Section~\ref{sec:sec:case-study}). If targeted enhancement of multi-hop analysis capability is needed, some existing question decomposition techniques~\cite{tang2026straptor} can be further applied.
% \end{R3Box}


% \noindent\ding{183} Second, we have added new experiments to compare MoDora and SHT on SHT's benchmarks and metrics, which shows that \oursys can not only handle queries in SHT's benchmarks, but also produce substantially higher quality when compared to the its results (see R2.O1 \ding{183}).

\begin{shaded*}
\noindent
\hypertarget{R2.O3-(1)}{\textbf{R2.O3-(1).}} The metric used is strange, it encourages long answers (e.g., returning the whole document as an answer gets ACNLS score of 100\% for any query). 
\end{shaded*}

\noindent \textbf{Response:} We thank the reviewer for the feedback. The reviewer is correct that evaluation metrics should not unfairly encourage long answers. To validate that ACNLS does not naively reward verbosity (i.e., by giving a perfect ACNLS 100\% score to when the entire document is returned as the answer), we conducted a control experiment in which a naive method always outputs the full document as its answer, in \lspref{whole_output} of our revised paper. This yields ACNLS scores of 43.85 and 64.72 on \ourbench and DUDE, both well below 100 and also lower than the scores that \oursys can achieve. These results indicate that ACNLS does not blindly favor longer responses, as many questions require non-trivial reasoning over the document rather than simple content inclusion.
%showing that ACNLS does not blindly reward longer responses. That's because many questions are not simple look-up ones and reasoning based on the document content are required to arrive at the correct answer.


We find the reviewer's idea of modifying ACNLS to punish verbose output quite interesting, so we followed the suggestion and  tested a modified metric, m-ACNLS, which scale ACNLS using a containment-style factor, based on the ratio of ``reference-answer length'' over ``model-answer length'', thereby explicitly penalizing verbose model answers (if a model's answer is substantially longer than the reference-answer, its m-ACNLS will be low).

We conducted an experiment using the modified m-ACNLS as the scoring metric, with a detailed comparison shown in \textbf{Table~\ref{tab:modify}}. We are happy to report that \oursys continues to dominate all other methods, outperforming other methods by at least 10 percentage points. We believe this modified metric can further strengthen our paper and we thank the reviewer for the helpful suggestion.

%while the scores of all methods drop in different degrees, \oursys still clearly outperforms all existing methods, showing its superiority under a variety of different possible metrics. Since the modification aims at punishing long outputs, DocAgent that generates answers with detailed explanations suffers the most decrease (about 15\%), \oursys with a few explanations in answers has ACNLS drop by about 5\%, and the rest drop by around 2\%. Since this experiment shows that the modified variant of ANCLS continues to show the strength of \oursys, we will include the modified ANCLS in the full version of our paper to further strengthen our results. We thank the reviewer for the helpful suggestion.
%this metric in the main text will still be calculated using the original definition.

Finally, in order to eliminate any doubt that MoDora's quality gains stem from the use of the ACNLS metric, in the revised paper 
we additionally report results using the precision and recall metrics, on the same datasets evaluated by SHT~\cite{sht}. As shown in {\emph{\textbf{Table~\ref{tab:sht}}}} and discussed in \hyperlink{R2.O1-(1)}{R2.O1-(1)}, MoDora consistently outperforms prior methods, under the traditional precision/recall metrics as well.

% \iffalse
% We thank the reviewer for the feedback. The reviewer is correct that evaluation metrics should not unfairly encourage long answers. % ACNLS metric was designed to mitigate false negatives when evaluating long-form LLM answers, particularly in cases where the annotated answers are short but the model generates longer, semantically similar content. 
% To validate that ACNLS does not naively favor verbosity (i.e., returning the whole document as an answer would yield an ACNLS score of 100\%), we conducted a control experiment in which the model outputs the full document as the answer. This yields ACNLS scores of 43.85 and 64.72 on our two benchmarks  (far below 100 and also lower than \oursys's original score 77.24 and 55.23), showing that ACNLS does not blindly reward longer responses. That's because many questions are not simple look-up ones and reasoning based on the document content are required to arrive at the correct answer.

% %This yields ACNLS scores of 43.85 and 64.72 on our two benchmarks (far below 100), showing that ACNLS does not blindly reward longer responses. %\xbr{on our datasets since they are not all look-up questions as 

% % \begin{R3Box}
% % \lspref{whole_output}
% %  To prove the effectiveness of ACNLS metric, we conduct an experiment that directly use the content of whole document as the answer. It result in 43.85 on \ourbench and 64.72 on DUDE, both much lower than the score of \oursys. It indicates that the advantage of \oursys comes from the retrieval and reasoning based on document content, instead of a special metric design and whole-document output.
% % \end{R3Box}

% To eliminate any concern that MoDora's quality gains stem from the use of the ACNLS metric, we have added experiments using the same precision/recall metrics as used in SHT. The new results, as discussed in R2.O1, confirm that MoDora continues to outperform prior methods under the precision/recall metrics.

% Besides, we find the reviewer's idea of modifying ACNLS to punish verbose output (e.g., by scaling with the reference-to-output length ratio) interesting, and conducted such an experiment as well. We are happy to report while the scores of all methods drop in different degrees, \oursys still clearly outperforms all existing methods, showing its superiority under a variety of different possible metrics. \xbr{Since the modification aims at punishing long outputs, DocAgent that generates answers with detailed explanations suffers the most decrease (about 15\%), \oursys with a few explanations in answers has ACNLS drop by about 5\%, and the rest drop by around 2\%. The detailed comparison is in Table~\ref{tab:modify}. Because this experiment demonstrates that the modification of ANCLS definition does not affect the main conclusion, this metric in the main text will still be calculated using the original definition.}
% \fi

\begin{table}[!t]
\centering
\caption{Comparison of ACNLS and modified-ACNLS on \ourbench.}
\label{tab:modify}
\vspace{-.5em}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c c c c c c c c}
\midrule
\textbf{Method} & \textbf{\oursys} & \textbf{GPT-5} & \textbf{M3DocRAG} & \textbf{Zendb} & \textbf{DocAgent}\\ \hline

ACNLS & 55.23	& 41.55 & 41.12 & 36.68 & 37.10\\
m-ACNLS	& 49.60	& 39.76	& 39.18	& 34.39 & 22.57\\
\bottomrule
\end{tabular}
\vspace{-1.5em}
\end{table}

\iffalse
\begin{R3Box}
\lspref{modify_acnls} 
(1) \textbf{ACNLS}: Since LLMs often produce additional contextual text in generated answers, the original ANLS~\cite{biten2019scene}, based on Levenshtein distance, may be penalized or lead to misjudgments. To address this, we assign a containment score to any prediction that contains the annotated answer, and its value is designed to be the reference-to-output length ratio to punish too long outputs. (2) \textbf{AIC-Acc}: We compute accuracy using LLM-based judgments (output 1 if the LLM determines the result is correct, otherwise 0). And we also give a score of 1 to generated answers that contain the annotated ground truth despite the LLM-based judgments to tolerate extraneous content, improving robustness to LLM verbosity.
\end{R3Box}

\zxh{replace with modified ACNLS throughout the paper?}
\fi

%Thanks for your concern and feedback about the ACNLS metric.  
%\noindent \ding{183} Second, you are correct that \textit{evaluation metrics should not unfairly encourage long answers}. To validate that ACNLS does not naively favor verbosity (i.e., returning the whole document as an answer would yield an ACNLS score of 100\%), we conducted a control experiment in which the model outputs the full document as the answer. 

%We find your idea of modifying ACNLS to punish verbose output (e.g., by scaling the 100\% containing score with the reference-to-output length ratio) interesting, and implement this change to the ACNLS score in the revised paper. We are happy to report while the score of all methods decrease slightly with the punishment, the relative rank of all methods stay the same (with MoDora still clearly outperforms all existing methods), showing the superiority of MoDora under a more reasonable metric.

%\noindent $\bullet$ \textbf{(1) Micro Benchmark Preparation(Section~\ref{ssec:bench}):} We have updated the definition of ACNLS in Section~\ref{ssec:bench}, where the long output is punished even it contains the annotated answer.



% \noindent $\bullet$ \textbf{(2) Experiments (Section~\ref{sec:experiments}):} We have updated the ACNLS score of all methods with the new definition.

\begin{shaded*}
\noindent
\hypertarget{R2.O3-(2)}{\textbf{R2.O3-(2).}}
The paper should discuss parameter settings for the baselines used and how many chunks were retrieved.
\end{shaded*}

\noindent \textbf{Response:} This is an excellent point. We have clarified the parameter settings in \lspref{parameter} and added detailed documentation for these parameters in the accompanying code repository~\cite{sht, docagent, m3raggit}, ensuring full reproducibility of our results.

Specifically, for baselines including SHT, we use the default parameter settings provided in their open-source repositories, and use GPT-5 as the underlying LLM API for all methods. For MoDora and TextRAG, the number of retrieved chunks is set to 3, while for SV-RAG and M3DocRAG, the number of retrieved pages is also 3.



% Thanks for your comments.
% For most baselines including SHT, we utilize default implementations and parameter settings in their open source repositories and uniformly apply GPT-5 as the LLM API. The retrieved chunks in MoDora are 3, and for SV-RAG and M3DocRAG, we set the number of retrieved pages to 3.

%Additionally, we have also compared \oursys with the officially results under the default settings in SHT's repository, which still shows improvements (see R2.O1).

% \noindent $\bullet$ \textbf{Experimental Setup (Section~\ref{subsec:setup}):} We have refined the description of model and parameter settings in Section~\ref{subsec:setup} to make them more clear.

% \begin{R3Box}
% \lspref{parameter} 
% We set $n_0=2$ and $k=2$ for bottom-up summarization, $temperature = 1$ for LLM generation, and the number of retrieved chunks by embedding search is 3. Other parameter settings for the baselines are the same as the default implementations in their open source repositories.
% \end{R3Box}


\begin{shaded*}
\noindent
\hypertarget{R2.O3-(3)}{\textbf{R2.O3-(3).}}
Removing tree-based retrieval leads to limited drops, meaning that the importance of the tree is unclear. In fact, without the tree, the method performs embedding search plus verification which is a standard rag set up and is unclear why that performs so much better than the baselines.
\end{shaded*}

\noindent \textbf{Response:} We thank the reviewer for raising this important point. We would like to clarify a potential confusion between the w/o tree-based retrieval variant and a standard RAG setup. The embedding retrieval variant in this ablation experiment \textit{still relies on part of the tree structure}, with each child node under the root as the chunk boundary, and further chunking within each node. The retrieval results also need to pass backward verification and are assigned the node path. Its performance actually verifies the important auxiliary role of tree structure and backward verification in RAG. In contrast, the TextRAG baseline is closer to the standard RAG set up you mentioned, and it performs over 25\% worse than \oursys on both MMDA and DUDE. 
We have refined the description of \oursys variants in \lspref{re_ablation}. 

%We apologize for the confusion but the w/o tree-based retrieval method in our ablation still uses node boundaries, paths and backward verification, which is why it shows a small drop – the TextRAG baseline is closer to the standard RAG, which is 25\% worse than \oursys.

%\noindent $\bullet$ \textbf{Ablation Study (Section~\ref{subsec:ablation}):} 

% \begin{R3Box}
% \lspref{re_ablation} We disable the LLM forward search, meaning that LLM is no longer used to choose nodes based on their titles and metadata. Instead, embedding search and backward verification are performed on the tree. Tree nodes continue to serve as chunk boundaries, node paths are still used to provide context, and the answering model maintains the chance to refer to the entire CCTree in cases where retrieval fails. This results in AIC-Acc drops of 5.3\% on DUDE and 2.44\% on \ourbench, indicating that the structure-aware tree-based retrieval contributes to improved performance.
% \end{R3Box}


\begin{shaded*}
\noindent
\hypertarget{R2.O3-(4)}{\textbf{R2.O3-(4).}} Finally, the queries in the benchmark do not seem realistic and are ambiguous. For example, the query ``what main aspects does the Discussion include?'' is unrealistic and it is unclear what the answer should be.
\end{shaded*}


\noindent \textbf{Response:} We would like to clarify that such questions (e.g., summarizing salient information from long documents) represent a common type of real-world questions,  that can also be found in prior studies and benchmarks too (e.g.,~\cite{zhang2025systematic}), and thus our evaluation is not unique in considering these questions that are common in practice. We have revised the description in \lspref{hier_query} to make this clearer.


While these questions can appear open-ended, the annotated reference answers are often not ambiguous (e.g., reference answers are often sub-titles or bold headers extracted from relevant sections of the document). %, and the correct answers are often not completely the same. 
For evaluation, although model responses may not exactly match reference answers, our proposed AIC-Acc and ACNLS metrics can reliably score answers based on semantic similarity. %(e.g., with the help of \llm assessment in the case of AIC-Acc). %, rather than exact string matching. 
%This allows the metrics to accommodate legitimate variations in wording, structure, and granularity across multiple valid answers. 
We have clarified this point in \lspref{open_end}.



%Thus, we design AIC-Acc and ACNLS to evaluate the answers to such questions (e.g., justified as positive if with the similar semantics with varied sentence structures, lexical choices, and levels of detail for any of the multiple ground-truth correct answers) (in \lspref{open_end}).  

% with multiple correct answers
%(see \hyperlink{R2.O3-(1)}{R2.O3-(1)} above).

%While such questions can be open-ended, the annotated answers are short key points (e.g., titles or bold headers) and the correct answers are often not completely the same, which AIC-Acc and ACNLS are designed to handle (see R2.O3-(1) above).

%The designs of such questions and the evaluation for open-ended questions have be clarified in  and \lspref{open_end}, respectively.

%\noindent $\bullet$ \textbf{(1) Semi-Structured Document Analysis (Section~\ref{subsec:questiontype}):} We have explained the usage scenarios of such questions to reflect their significance in Section~\ref{subsec:questiontype}.

% \begin{R3Box}
% \lspref{hier_query}
% \xbr{The target of such tasks lies in extracting key titles or summaries from multiple document sections, as opposed to retrieving detailed paragraph contents.
% }
% \end{R3Box}

% % \noindent $\bullet$ \textbf{(2) Micro Benchmark Preparation(Section~\ref{ssec:bench}):} We have explained the design of the two metrics to accommodate open-ended questions that lack uniquely determined answers.

% \begin{R3Box}
% \lspref{open_end}
% %Given that the datasets used predominantly consist of open-ended questions, \zxh{our metric design integrates edit distance, LLM-based assessment, and string containment} to comprehensively evaluate response quality, rather than relying on simplistic exact-match judgments.
% For such open-ended queries (about 15\% in \ourbench), we adopt approximate evaluation for such cases, where annotated answers are short but concise key points (e.g., section titles or bold headers). Instead of requiring exact matches, we compute the edit distance between the predicted and gold answers and assess quality using our proposed metrics (AIC-Acc and ACNLS), which are designed to tolerate semantically correct but lexically varied answers.
% \end{R3Box}


%we support approximate evaluation to support correct answers that are often not completely the same. Specifically, the annotated answers for these queries are short key points (e.g., titles or bold headers) and, given an answer, we compute its edit distance with the answer, which is measured by the proposed metrics (AIC-Acc and ACNLS) to ensure xxx


% While such questions can be open-ended, the annotated answers are short key points (e.g., titles or bold headers), and the correct answers are often not completely the same, which AIC-Acc and ACNLS are designed to handle (see R2.O3-(1) above).


\section*{Response to Reviewer \#3 \textcolor{red}{(Red)}}

\iffalse
\begin{table}[h]
\vspace{-.3cm}
\caption{Revision Summary for Reviewer \#3.}
\vspace{-.35cm}
\label{tab:reviewer2}
\resizebox{.95\linewidth}{!}{
\begin{tabular}{c|l|c}
\hline
\textbf{ID} & \multicolumn{1}{c|}{\textbf{Revision Items}} & \textbf{Requests} \\ \hline
\textbf{1}  & Evaluate the cost of LLM-based approaches and \oursys's modules.  & R3.O1 \\ \hline
\textbf{2}  & Add a baseline excluding the tree-based optimizations in Section~\ref{subsec:ablation}. & R3.O2 \\ \hline
\textbf{3}  & Report the tree statistics like the size to prove its necessity in Section~\ref{ssec:bench}.  & R3.O3 \\ \hline
\textbf{4}  & Clarify the LLM question generation and manual curation in Section~\ref{ssec:bench}.  & R3.O4 \\ \hline
\textbf{5}  & Discuss the performance of LLMs to generate captions/metadata. & R3.O5\\ \hline
\end{tabular}
}
\vspace{-.25cm}
\end{table}
\fi

%\vspace{2em}

\begin{shaded*}
\noindent
\hypertarget{R3.O1}{\textbf{R3.O1.}} The cost overhead of the approach seems significantly high. The method requires multiple calls to an MLLM and an LLM, making the dollar cost of using GPT-5 high. There needs to be an experiment compares the costs, and also breaks down the cost of different stages.
%for each extracted component through various stages of the pipeline. The dollar cost of this approach using a pay-per-use model like GPT-5 is likely prohibitively high. There needs to be an experiment which compares the costs of these approaches and also breaks down the cost of different stages of the pipeline, including preprocessing, tree generation, and querying, in both dollar API costs (since the approach relies on powerful MLLM backbones) and the number of calls incurred at each stage.
\end{shaded*}

\begin{sloppypar}
\noindent \textbf{Response:} We thank the reviewer for the insightful comment and agree that this would be an important analysis of our study. We have added a detailed cost analysis of \oursys in \lspref{cost}. The average cost of \oursys (applying local-model-offloading optimization) is \$0.025 per query, comparable to other baselines (e.g. GPT-5 at \$0.01 per query, and DocAgent at \$0.09 per query), but achieves over 15\% higher accuracy than them.

For API-based LLM calls, by offloading relatively simple operations to local models, \oursys needs 1 calls for preprocessing, 0 for tree construction, and 4 for analysis. {For
API token usage, the preprocessing needs 369k prompt tokens and 1084k completion tokens to process the whole \ourbench dataset, while analysis needs 6654k prompt tokens and 604k completion tokens. We have clarified the API costs of \oursys's stages and other two approaches in {\emph{\textbf{Table~\ref{tab:cost}}}}.}

%14 calls for preprocessing, 23 for tree construction, and 8 for analysis respectively for each query in average; but , these can be reduced to 1, 0, and 4 API-based calls, respectively, leading to a great reduction in cost. 


% \begin{R4Box}
% \lspref{model_setup}
% We employ PaddleOCR~\cite{cui2025paddleocr30technicalreport} for detecting elements within documents and Qwen3-Embedding-8B~\cite{qwen3embedding} for embedding search. For relatively simple tasks including information enrichment, summarization generation, forward search and backward verification, we locally implement Qwen2.5-VL-7B-Instruct~\cite{qwen2.5-VL}. GPT-5 is applied for more challenging tasks including hierarchy detection, question parsing and final question answering in \oursys, as well as the uniformly external LLM-API for baselines.
% \end{R4Box}
\end{sloppypar}

% \begin{R4Box}
% \lspref{cost} 
% % We compare the costs of \oursys with \zxh{xxx -- list detailed baseline names}. 
% % For the api-key employed in our study (priced at \$1.25 per million tokens for prompts and \$10 per million tokens for completions) amounting to approximately \$10 in cost, 
% %To reduce dollar costs, \oursys offloads simple sub-tasks (e.g., information enrichment, and summarization) to locally deployed open-source models, while sending the remaining more challenging steps to GPT-5, to further reduce \oursys's cost. For example, on average \oursys makes 14, 23, and 8 LLM calls for preprocessing, tree construction, and querying, respectively, which can be reduced to 1, 0, and 6, respectively, by offloading the aforementioned simpler tasks to local open-source models, therefore significantly reducing costs by 6x. We will discuss these cost optimizations in detail in our revised paper.
% For \ourbench, by applying local-model-offloading optimization (see Section~\ref{subsec:setup}), \oursys via GPT-5 consumes a total of 6,654k prompt tokens and 604k completion tokens (where the former is much cheaper than latter), with an average cost of \$0.025 per query. By contrast, directly invoking GPT-5 uses 771k prompt tokens and 876k completion tokens, at an average cost of \$0.01 per query. In this way, we avoid the substantially higher costs of \oursys while still achieving markedly better performance than the baseline (over 25\% higher accuracy, as detailed in Section~\ref{subsec:overallperformance}). Concretely, for \ourbench, \oursys typically issues 14, 23, and 8 LLM calls for preprocessing, tree construction, and querying, respectively; but by offloading the aforementioned simpler operations to local open-source models, \xbr{these can be reduced to 1, 0, and 4 API-based LLM calls, respectively, leading to a great reduction in cost.} % Thus the cost of \oursys is comparable with simpler baselines, but achieves much higher accuracy (e.g. 25\% more than GPT-5 on \ourbench).
% % The reason is that \oursys can offload simple sub-tasks (e.g., information enrichment, and summarization) to locally deployed open-source models, reserving only the more difficult steps for GPT-5.
% \end{R4Box}


%\noindent\ding{182} First, we would like to clarify that our average cost is \$0.05 per document, comparable with other GPT-5 based methods tested in our experiments, but achieves over 25\% higher accuracy.

%\noindent\ding{183} Second, \oursys can actually offload simple sub-tasks (e.g., information enrichment and summarization) to locally deployed open-source models, while sending the remaining more challenging steps to GPT-5, to further reduce our cost.

%\noindent $\bullet$ \textbf{Experimental Setup (Section~\ref{subsec:setup}):} We have clarified the model used for each step in Section~\ref{subsec:setup}.

%\noindent\ding{184} Third, we added an experiment to compare the costs of \oursys and some baselines, as well as break down the cost of different stages of \oursys.

%\noindent $\bullet$ \textbf{Fine-Grained Result Analysis (Section~\ref{subsec:finegrained}):} We have add the experimental results about the cost of LLM API in Section~\ref{subsec:finegrained}.


\begin{shaded*}
\noindent
\hypertarget{R3.O2}{\textbf{R3.O2.}} It is necessary to add a baseline that just uses the extracted components to prompt the MLLM with the same retrieval strategies as the current approach (excluding the tree-based optimizations). This would help isolate whether the gains come from the element aggregation step that generates rich layout-aware components versus the tree-based approach itself.
\end{shaded*}

\noindent \textbf{Response:} We agree that this is an excellent suggestion, and added such a baseline for \oursys without tree-based optimizations (see {\emph{\textbf{Table~\ref{tab:ablation}}}} and \lspref{hi_ablation}), which shows a significant drop in quality -- e.g., (73.33 -> 59.25), (55.23 -> 45.85) for AIC-Acc and ACNLS on MMDA, and (83.70 -> 68.86), (77.24 -> 62.96) for the same on DUDE, respectively. This new ablation indeed underlines the importance of the tree-based optimization and strengthens our paper.

% Thanks for your valuable suggestion.
% We have conducted such an experiment. There is a significant drop in quality (73.33 -> 57.84), (55.23 -> 44.23) for AIC-Acc and ACNLS on MMDA, and (83.70 -> 68.37) (77.24 -> 63.97) for the same on DUDE, which underlines the importance of the hierarchical representation in \oursys.

% \noindent $\bullet$ \textbf{Ablation Study (Section~\ref{subsec:ablation}):} We have add the experimental results of the suggested baseline in Section~\ref{subsec:ablation}.

% \begin{R4Box}
% \lspref{hi_ablation} We isolate the impact of hierarchical representation via conducting question answering based on the flattened components with the same retrieval strategies. Without the assistance of tree structure, the AIC-Acc decreases greatly by -15.33\% and -15.49\% on DUDE and \oursys respectively. This demonstrates the utility of our structural modeling of CCTree.
% \end{R4Box}


\begin{shaded*}
\noindent
\hypertarget{R3.O3}{\textbf{R3.O3.}}  It is also necessary to discuss/show what is the size of the generated trees for real-world semi-structured documents. For the documents in the provided dataset, the generated trees do not seem too complex. The expensive tree-based approach seems unnecessary for these documents.
\end{shaded*}

\noindent \textbf{Response:} We thank the reviewer for the comment. In the existing DUDE benchmark, the average document tree contains 17.2 nodes, 12.6 leaves, and 3.36 hierarchical levels. In contrast, the newly introduced MMDA benchmark exhibits substantially higher complexity, with an average of 49.2 nodes, 37.7 leaves, and 4.23 levels. We now explicitly report these statistics in {\emph{\textbf{Table~\ref{tab:datasets}}}} and discuss them in \lspref{dataset_cmp}. These results highlight the significantly increased structural complexity of the documents, motivating the need for explicit hierarchical modeling of elements such as section headers, nested lists, and grouped visual components. Such tree-based structural representations enable more accurate summarization and more effective forward search during answer retrieval.

To further demonstrate this point, our ablation study in \hyperlink{R3.O2}{R3.O2} demonstrates that a significant 15 percentage point performance drop when this tree structure is removed  (see {\emph{\textbf{Table~\ref{tab:ablation}}}}), confirming its utility. %Additionally, as shown in our response to \hyperlink{R3.O1}{R3.O1}, the computational cost of the tree-based approach remains comparable to other retrieval methods like shown in {\emph{\textbf{Table~\ref{tab:cost}}}}, making it a practical and impactful design choice.


%We appreciate the reviewer's suggestion. To address this, we analyzed the complexity of the generated trees across benchmarks in {\emph{\textbf{Table~\ref{tab:datasets}}}}. In the existing DUDE dataset, the average tree contains 17.2 nodes, 12.6 leaves, and 3.36 levels. In contrast, our newly constructed MMDA benchmark yields significantly more complex trees, with 49.2 nodes, 37.7 leaves, and 4.23 levels on average. This increase in structural richness reflects the greater layout and content complexity of MMDA documents, reinforcing its value as a more challenging benchmark for DocumentQA.

%The motivation for adopting a tree-based structure lies in its ability to 

%We thank the reviewer for the suggestion -- in the existing DUDE benchmark, the average tree size is 17.2 nodes, 12.6 leaves and 3.36 levels; while in the new MMDA benchmark we create, the numbers are 49.2 nodes, 37.7 leaves and 4.23 levels, respectively. This shows greater complexity of documents in MMDA, making MMDA a more challenging DocumentQA benchmark, which is as another valuable contribution of this work. We have added comparison of tree complexity  among different datasets of semi-structured documents in Section~\ref{ssec:bench}.


%We apply tree structure for these documents since it naturally captures hierarchical relationships within documents, such as heading levels. Building upon this structure, summarization generation and forward search further enable effective retrieval. The ablation study in R3.O2 has shown a 15\% drop without this structure, indicating the importance of tree representation in document modeling. And the experiment for R3.O1 also shows the cost for tree-based approach is comparable to some others.

% \noindent $\bullet$ \textbf{Micro Benchmark Preparation(Section~\ref{ssec:bench}):} We have calculated the dataset statistics such as the LD, ED and tree size. They are reported in Section~\ref{ssec:bench} to prove the complexity of \ourbench compared to other datasets, further indicating the necessity of tree construction.

% \begin{R4Box}
% % \lspref{dataset_ana} Existing datasets cannot well reflect the complexity of typical semi-structured document analysis tasks~\cite{tito2023hierarchical,cho2024m3docrag,van2023document}. The documents in MP-DocVQA~\cite{tito2023hierarchical} and DUDE~\cite{van2023document} exhibit limitations in content sufficiency, element richness and structural complexity. While M3DocVQA~\cite{cho2024m3docrag} is more challenging in these aspects, its documents are sourced from Wikipedia, lacking representativeness of other types of complex documents. Thus, in this section we introduce a new benchmark \oursys.
% \lspref{dataset_cmp} Besides, we compute various statistics for the four datasets, including the previously defined ED and LD, as well as the average number of nodes, leaves and levels of the CCTree constructed based on their documents. As shown in Table~\ref{tab:datasets}, \ourbench achieves lower ED (0.264 compared to 0.305 of MP-DocVQA), higher LD (1.85 compared to 1.35 of DUDE) and more tree nodes (49.2 compared to 38.3 of M3DocVQA). These optimal statistics indicate its richer document element types, complexity of layout distribution, and sufficiency of content. \ourbench has fewer average CCTree levels than M3DocVQA, which is partly attributable to the fact that M3DocVQA consists of Wikipedia documents, which inherently possess more hierarchical title levels, whereas \ourbench also encompasses some document types with fewer heading levels.
% \end{R4Box}


\begin{shaded*}
\noindent
\hypertarget{R3.O4}{\textbf{R3.O4.}} The question generation for the MMDA benchmark uses an LLM to generate the QA pairs. Given that the LLM's (e.g. GPT-5) inability to process complex structures is the primary motivation of the paper, the LLM-generated questions could be sub-optimal for testing the benchmark suite which contains such complex layouts. It would be beneficial to know how the LLM-generated questions in the benchmark were manually curated to overcome this limitation.
\end{shaded*}

\noindent \textbf{Response:}
Thank you for raising this important point. While GPT-5 may not excel at answering questions over complex documents, it is well suited for generating realistic questions—an observation aligned with prior work showing that question generation is generally easier than question answering (e.g.,~\cite{chen2024sv}). We prompt GPT-5 with carefully designed question templates to ensure both diversity and accuracy, and all generated questions are then carefully reviewed by multiple human annotators. Defective QA pairs are revised through manual curation, with particular attention to cases requiring structural understanding or content-intensive reasoning. We have added additional details in \lspref{qa_curation} to clarify how this human-in-the-loop process ensures the quality of the generated document questions.

% While results show GPT-5 does not excel at answering complex document questions, it is well-suited for generating complex and representative ones. We prompt it using question templates to ensure diversity and accuracy, and further manually review all outputs. Defective QA pairs are revised by human annotators, prioritizing those involving structural or content-intensive reasoning.

%\noindent $\bullet$ \textbf{Micro Benchmark Preparation(Section~\ref{ssec:bench}):} We have refined the introduction of the LLM question generation and manual curation in Section~\ref{ssec:bench} to better reflect the question quality.

% \begin{R4Box}
% \lspref{qa_curation}
% \xbr{Given GPT-5's excellent instruction-following ability and a certain degree of document comprehension capability, we employ it to generate question-answer(QA) pairs. We first craft instructions and few-shot examples for each defined task type, and further distinguishing between look-up questions and multi-hop questions. We then randomly sample question types according to a preset ratio, prompting GPT-5 to generate similar questions by adhering to the corresponding instructions and examples. The generated QA pairs are then checked and refined by humans.}
% During the rewriting of defective questions, human annotators prioritize crafting multi-hop queries that require complex structural and content-based reasoning. All QA pairs after rewriting are finally checked again for the correctness.
% \end{R4Box}


\begin{shaded*}
\noindent
\hypertarget{R3.O5}{\textbf{R3.O5.}} The template-based information enrichment process uses an expensive MLLM to add LLM-generated captions/metadata to non-textual elements. Would this not generate hallucinations from the model especially if the required context for the caption is available in surrounding text that is not present in the current component?
\end{shaded*}

\noindent \textbf{Response:} This is a great question. Empirically, in our manual analysis, only 3\% of enriched outputs contain hallucinated content (see our revised \lspref{vl_error}). We minimize the risk of hallucinations, by applying heuristic rules to match non-textual elements against existing captions; if a match is found, we skip generation altogether, thereby avoiding the risk of hallucination. Otherwise, we invoke a template-based prompt tailored to the element type (e.g., tables, charts, etc.), using few-shot examples to guide MLLM in generating reliable captions and metadata. Since each component is a self-contained group of interrelated elements, visual and contextual information within the component is typically sufficient for accurate description. Lastly, the enrichment step is performed using a locally deployed, cost-efficient model rather than relying on expensive APIs (please see our revised \lspref{model_setup} for clarification).


% During the integration of elements into components, we first apply rules to match existed captions; when a match is found, the generated caption is not used. Otherwise, we construct type-specific prompts (e.g. different few-shot examples for tables, charts and images) to instruct the MLLM to generate description including caption and metadata. Because each component is a self-contained group of document elements, description over the component image suffices to recover information of non-textual elements. Empirically, we observe that only 3\% of cases exhibit erroneous content descriptions attributable to hallucinations (see \lspref{vl_error}). Notably, this result is achieved using a cost-effective, locally deployed model rather than expensive API calls (see \lspref{model_setup}).


%Captions for non-textual elements often encode information grounded directly in the visual content, forming self-contained components that are typically sufficient for tree-based LLM reasoning. To reduce hallucinations, we prompt the MLLM to describe rather than interpret visual input \yeye{describe vs. interpret -- the difference is not very clear}. Surrounding textual context is preserved via edges linking text and non-text nodes during tree construction stage, and is further leveraged during data search.


%Empirically, \oursys achieves high reliability in this step, with well summarized captions and metadata for more than 97\% non-textual elements \yeye{can we be more specific, how did we get this 97\% number, so that it can be more convincing? I did not find this 97\% number in the revised paper, add?}. We have clarified the design and safeguards of our caption generation process in \lspref{hallu} and reported empirical statistics on hallucination frequency (this type of error occurs in only approximately 3\% of the generated results \zxh{and \oursys can still correctly answer for these 3\% because xxx}) in \lspref{vl_error}.

% \begin{R4Box}
% \lspref{hallu}
% \xbr{Since such a component is a self-contained unit of a table/chart/image and its possibly existed title, \llm have sufficient information when describing its content and can avoid hallucinations in most cases.}
% \end{R4Box}

%Thanks for your question. We find captions for non-textual elements often encode information grounded directly in the visual content, forming self-contained components that are typically sufficient for tree-based LLM reasoning. To reduce hallucinations, we prompt the MLLM to describe rather than interpret visual input. Surrounding textual context is preserved via edges linking text and non-text nodes during tree construction stage, and is further leveraged during data search.  Furthermore, we manually examined the intermediate results of information enrichment to assess the reliability of this process. Empirically, \oursys achieves high reliability in this step, with well summarized captions and metadata for more than 97\% non-textual elements.

% \noindent $\bullet$ \textbf{Fine-Grained Result Analysis (Section~\ref{subsec:finegrained}):}  We have added the manual observation of the LLM captions/metadata generation performance in Section~\ref{subsec:finegrained}.




% \begin{R4Box}
% \lspref{vl_error}In addition to structural errors, information enrichment may also generate incorrect descriptions of images, tables, charts, and propagate such errors into the content of tree nodes. By manual observation, we found such error occur in only approximately 3\% of the generated results, indicating that it is not a major factor affecting the validity of the tree.
% \end{R4Box}



\begin{shaded*}
\noindent
\hypertarget{R3.M1}{\textbf{R3.M1.}}  Writing nits.

% -- Section 8.2: “This design can benefit the subsequent tree construction and analysis operate at a fine-grained yet complete level.”

% -- Section 8.2: “thereby facilitating accurate and efficient information retrieval for QA tasks like over documents with multi-level nested structures (four level in general)”

% -- Section 8.3: ``Manual observation shows the selector and embedding search recall all required evidence with 91\%''
\end{shaded*}

\noindent \textbf{Response:}
Thank you for pointing these out. We have carefully proofread our paper and fixed these and other minor writing issues. %The corrections are as follows: 

% This design can benefit the subsequent tree construction and analysis operate at a fine-grained yet complete level. -> This design benefits the subsequent tree construction and analysis, enabling them to operate at a fine-grained yet complete level.

% thereby facilitating accurate and efficient information retrieval for QA tasks like over documents with multi-level nested structures (four level in general) -> thereby facilitating accurate and efficient retrieval from documents with multi-level nested structures

% Manual observation shows the selector and embedding search recall all required evidence with 91\% -> Manual observation reveals that the selector and embedding search recall all required evidence with a rate of 91\%
